Peak Estimation for Uncertain and Switched Systems

Peak estimation bounds extreme values of a function of state along trajectories of a dynamical system. This paper focuses on extending peak estimation to continuous and discrete settings with time-independent and time-dependent uncertainty. Techniques from optimal control are used to incorporate uncertainty into an existing occupation measure-based peak estimation framework, which includes special consideration for handling switching uncertainties. The resulting infinite-dimensional linear programs can be solved approximately with Linear Matrix Inequalities arising from the moment-SOS hierarchy.

==> sections/affine.tex <==
\section{Affine Uncertainty}

\label{sec:affine}

Many dynamical systems exhibit a input-affine or parameter-affine structure:

\begin{equation}
\label{eq:affine_base}
    \dot{x} = f(t,x,w) = f_0(t,x,w) + \sum_{w=1}^{N_w} w_k f_k(t,x,w)
\end{equation}

Peak estimation of input-affine systems with time-varying uncertainty may proceed through the methods of Problem \eqref{eq:peak_meas_w} and \eqref{eq:peak_cont_w}. In some specific cases where there are no moment constraints $h(w)$, the affine structure may drastically simplify computation.

\cite{majumdar2014convex, korda2014controller}



\subsection{Polytopic Uncertainty}
\label{sec:polytopic}

Polytopic uncertainty is an instance of time-varying uncertainty where all $w_i \geq 0$ and $\sum_i w_i = 1$. The dynamics from equation \eqref{eq:affine_base} may be divided into:
\begin{equation}
\label{sec:poly_split}
    \sum_{w=1}^{N_w} w_k (f_0(t,x,w) + f_k(t,x,w) ) = \sum_{w=1}^{N_w} w_k \tilde{f}_k(t,x,w)
\end{equation}
for merged dynamics $\tilde{f}_k(t,x,w)$ on each parameter $w_k$. Dynamics in $f$ at every point in time are convex combinations of $\tilde{f}_k(t,x,w)$. Mixed dynamics may be realized as a system switching arbitrarily fast between base dynamics $\tilde{f}_k(t,x,w)$. 

A polytopic-uncertain system can be certified as stable if all components $\tilde{f}_k(t,x,w)$ have a common Lyapunov function \cite{parrilo2008approximation, vlassis2014polytopic}. In the same manner, the Function problem of peak estimation may be adapted to polytopic uncertainty by ensuring that the value function $v(t,x)$ satisfies:
\begin{equation}
    \Lie_{\tilde{f}_k} v(t, x) \geq 0 \quad \forall (t, x) \in [0, T] \times X, \ k=1\ldots N_w \label{eq:peak_cont_f_poly}
\end{equation}
Constraint \eqref{eq:peak_cont_f_poly} replaces constraint \eqref{eq:peak_cont_f} and constraint \eqref{eq:peak_cont_w_f}. The occupation measure $\mu$ and adjoint Lie derivative of constraint \eqref{eq:peak_meas_flow} can be decomposed into:
\begin{equation}
    \mu = \sum_k \mu_k \qquad \Lie^\dagger \mu = \sum_k \Lie^\dagger_{\tilde{f}_k} \mu_k
\end{equation}



The moments $\inp{t}{\mu_k}$ are the expected amount of time that trajectories spend following dynamics $\tilde{f}_k$. The switching sequence $w^*(t)$ connecting the optimal $x_0^* \rightarrow x_p^*$ is not immediately available from the truncated moments of all $\mu_k$, and requires postprocessing by the methods \cite{marx2019tractable} to recover.


Using the approach in \eqref{eq:peak_cont_w} results in one occupation measure $\mu$ with $n + N_w$ variables. With polytopic uncertainty, the $N_w$ occupation measures $\mu_k \in \Mp{[0, T] \times X}$ each have $n$ variables and do not involve $w$. The complexity of the moment-SOS hierarchy scales polynomially on the number of states and linearly on the number of measures, so depending on the degree $d$ it may be favorable to solve peak estimation in switched or polytopic form.



\subsection{Box Uncertainty}
\label{sec:box}
% All parameters are in a box

Box uncertainty is a case where each time-varying $w_k \in [w_k^{min}, w_k^{max}]$ with no other constraints on $w$. With a proper scaling of dynamics, all $w$ can be constrained to the region $w_k \in [0,1]$. The methods in \cite{majumdar2014convex, korda2014controller} introduce parameter-measures $\{\sigma_k \in \Mp{[0,T] \times X} \}_{k=1}^{N_w}$ such that  for all subsets $A \times B \in [0, T] \times X$.
\begin{equation}
    \int_{A\times B} w_k(t) d \mu(t,x) = \int_{A \times B} d \sigma(t,x)
\end{equation}
The peak estimation with box uncertainty in $[0, 1]^{N_w}$ is:
\begin{subequations}
\label{eq:peak_meas_box}
\begin{align}
p^* = & \ \textrm{max} \quad \inp{p(x)}{\mu_p} & \label{eq:peak_meas_box_obj} \\
    & \mu_p = \delta_0 \otimes\mu_0 + \Lie_{f_0}^\dagger \mu + \sum_{k = 1}^{N_w} \Lie_{f_k}^\dagger \sigma_k & \label{eq:peak_meas_box_flow}\\
    & \mu_0(X_0) = 1 & \label{eq:peak_meas_box_prob}\\
    & \sigma_k + \hat{\sigma}_k = \mu &\forall k = 1 \ldots N_w \label{eq:peak_meas_box_cont}\\
    & \sigma_{k}, \ \hat{\sigma}_k \in \Mp{[0, T] \times X} &\forall k = 1 \ldots N_w\\
    & \mu, \mu_p \in \Mp{[0, T] \times X}&\\
    & \mu_0 \in \Mp{X_0}& \label{eq:peak_meas_box_init}
\end{align}
\end{subequations}
Constraint \eqref{eq:peak_meas_box_flow} splits up dynamics in \eqref{eq:peak_meas_w_flow} across $\sigma_k$. Absolute continuity of $\sigma_k$ with respect to $\mu$ is enforced by constraint \eqref{eq:peak_meas_box_cont}. The dual program of \eqref{eq:peak_meas_box} is:
\begin{subequations}
\label{eq:peak_cont_box}
\begin{align}
    d^* = & \ \min_{\gamma \in \R} \quad \gamma & \\
    & v(0, x) + \gamma \geq 0  &  \forall x \in X_0 \label{eq:peak_cont_init_box}\\
    & \Lie_{f_0} v(t, x) \geq \sum_{k=1}^{N_w}\zeta_k(t,x)  & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_f_box}\\
    & \Lie_{f_k} v(t, x) + \zeta_k(t,x) \geq 0  & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_f_box}\\
    & v(t, x) + p(x) \leq 0 & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_p_box} \\
    & v \in C^1([0, T] \times X) & \\
    & \zeta_k \in C_+([0, T] \times X) & \forall k = 1 \ldots N_w
\end{align}
\end{subequations}

% The nonnegative functions  $\zeta_k$

    % & \Lie_{f_0} v(t, x) - \sum_{k=1}^{N_w}\zeta_k(t,x) \geq 0 & \forall (t, x) \in [0, T] \times X 
    % & \Lie_{f_k} v(t, x) + \zeta_k(t,x) \geq 0 & \forall k = 1 \ldots N_w, \ (t, x) \in [0, T] \times X \label{eq:peak_cont_f_box}\\
    % \zeta_k(t,x) \geq 0 & \forall k = 1 \ldots N_w, \ (t, x) \in [0, T] \times X \label{eq:peak_cont_f_box}\\
    % & v(t, x) + p(x) \leq 0 & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_p_box} \\
    % & v \in C^1([0, T] \times X) & \\
    % & \zeta_k \in C([0, T] \times X) & \forall k = 1 \ldots N_w\\

A system with $N_w$ parameters with box uncertainty from Section \eqref{sec:box} may be expressed as an instance of polytopic uncertainty with $2^{N_w}$ subsystems. Each subsystem is comprised of dynamics $\dot{x} = f_w(t,x)= f(t, x, w)$ where $w$ is fixed to a vertex of the box $W = \prod_{\ell=1}^{N_w} [0, \bar{w}_\ell]$. Since the number of subsystems (and measures) scale exponentially in $N_w$,  posing boxed uncertainty according to Section \eqref{sec:box} is generally more tractable than solving as a per-vertex switched system.


==> sections/affine_basic.tex <==
\subsection{Affine Uncertainty}

\label{sec:affine}

Many dynamical systems exhibit an affine structure in terms of the disturbance $d \in \Delta$:
\begin{equation}
\label{eq:affine_base}
    \dot{x} = f(t,x,d) = f_0(t,x,d) + \sum_{k=1}^{N_d} d_k(t) f_k(t,x,d)
\end{equation}
% Peak estimation of input-affine systems with time-varying uncertainty may proceed through the methods of Problem \eqref{eq:peak_meas_w} and \eqref{eq:peak_cont_w}. 
In some specific cases the affine structure may be used to simplify computation
\cite{majumdar2014convex, korda2014controller}.
\subsubsection{Polytopic Uncertainty}
\label{sec:polytopic}

Polytopic uncertainty is an instance of time-varying uncertainty where all $d_i(t) \geq 0$ and $\sum_i d_i(t) = 1$. The dynamics from \eqref{eq:affine_base} may be divided into:
\begin{equation}
\label{sec:poly_split}
    \sum_{k=1}^{N_d} d_k(t) (f_0(t,x,d) + f_k(t,x,d) ) = \sum_{w=1}^{N_w} d_k(t) \tilde{f}_k(t,x,d)
\end{equation}
for merged dynamics $\tilde{f}_k(t,x,w)$ on each parameter $w_k$. Dynamics in $f$ are convex combinations of $\tilde{f}_k(t,x,d)$. Mixed dynamics may be realized as a system switching arbitrarily quickly between base dynamics $\tilde{f}_k(t,x,d)$. The occupation measure $\mu \in \Mp{[0, T]\times X}$ and adjoint Lie derivative of constraint \eqref{eq:peak_meas_flow} can be decomposed \cite{henrion2012measures},
\begin{equation}
\label{eq:occ_poly}
    \mu = \textstyle\sum_k \mu_k \qquad \Lie^\dagger \mu = \textstyle\sum_k \Lie^\dagger_{\tilde{f}_k} \mu_k
\end{equation}
A valid auxiliary function $v(t,x)$ from \eqref{eq:peak_cont_f} must decrease along all subsystems \cite{parrilo2008approximation, vlassis2014polytopic}.
\begin{equation}
    \Lie_{\tilde{f}_k} v(t, x) \leq 0 \quad \forall (t, x) \in [0, T] \times X, \ k=1\ldots N_d \label{eq:peak_cont_f_poly}
\end{equation}
The moments $\inp{1}{\mu_k}$ are the expected amount of time that trajectories spend following dynamics $\tilde{f}_k$. 


% The switching sequence $w^*(t)$ connecting the optimal $x_0^* \rightarrow x_p^*$ is not immediately available from the truncated moments of all $\mu_k$, and requires postprocessing by the methods \cite{marx2019tractable} to recover.
% Using a time-dependent uncertainty approach in results in one disturbance-occupation measure $\mu$ with $n + N_d$ variables. With polytopic uncertainty, the $N_d$ occupation measures $\mu_k \in \Mp{[0, T] \times X}$ each have $n$ variables and do not involve $d$. The complexity of the moment-SOS hierarchy scales polynomially on the number of states and linearly on the number of measures, so depending on the relaxation degree it may be favorable to solve peak estimation in switched or polytopic form.

\subsubsection{Switching Uncertainty}
\label{sec:switching}
Switching uncertainty is a generalization of polytopic uncertainty.
Let $\{X^k\}_{k=1}^{N_s}$ be a closed cover of $X$ for $k=1\ldots N_s$, which is a set of not necessarily disjoint closed subsets $X^k \subseteq X$ such that $\cup_k X^k = X$. Further, let $\dot{x} = \tilde{f}_k(t,x)$ be dynamics that evolve on each $X_k$. 
The closed cover formalism generalizes partitions of $X$ where $X^k \cap X^{k'} = \varnothing \ \forall k \neq k'$ and arbitrary switching where $X^k = X \ \forall k$. The switched measure program introduces an occupation measure $\mu_k \in \Mp{[0, T] \times X^k}$ for each subsystem $\tilde{f}_k$ subject to \eqref{eq:occ_poly}. The nonnegativity condition \eqref{eq:peak_cont_f_poly} in $v(t,x)$ is restricted to each region $[0, T] \times X_k$
\begin{equation}
    \Lie_{\tilde{f}_k} v(t, x) \leq 0 \quad \forall (t, x) \in [0, T] \times X_k, \ k=1\ldots N_d \label{eq:peak_cont_f_switch}
\end{equation}

\subsubsection{Box Uncertainty}
\label{sec:box}
% All parameters are in a box

Box uncertainty is a case where the region $\Delta$ is a box, and there are no other constraints on $d(t)$. With a proper scaling of dynamics, all $d$ can be constrained to the region $d_k(t) \in [0,1]$. The methods in \cite{korda2014controller, majumdar2014convex} introduce box-measures $\{\sigma_k \in \Mp{[0,T] \times X} \}_{k=1}^{N_d}$ such that for all subsets $A \times B \in [0, T] \times X$.
\begin{equation}
    \int_{A\times B} d_k(t) d \mu = \int_{A \times B} d \sigma
\end{equation}

Each measure $\sigma_k$ is absolutely continuous with respect to the occupation measure $\mu$ $(\sigma(A \times B) \leq \mu(A \times B), \ \forall A \in [0, T], \ \forall B \in X$. It therefore holds that there exists a nonnegative measure $\hat{\sigma}_k \in \Mp{[0, T] \times X}$ such that $\sigma_k + \hat{\sigma}_k = \mu$ for each $k$.

% By the Jordan decomposition there exists nonnegative complement measures $\hat{\sigma}_k \in \Mp{[0,T] \times X}$ such that $\sigma_k + \hat{\sigma}_k = \mu$ for each $k = 1, \ldots, N_d$. 

The Liouville equation \eqref{eq:liou_d} may be expressed in terms of $\sigma$ for all test functions $v (t, x) \in C^1([0, T] \times X)$ as
\begin{equation}
    \inp{v(t, x)} {\mu_p} = \inp{v(0, x)}{\mu_0} + \inp{\Lie_{f_0}  v(t, x)}{\mu} + + \textstyle\sum_{k = 1}^{N_w} \inp{f_k \cdot \nabla_x v (t,x)}{ \sigma_k}
\end{equation}
\begin{equation}
\label{eq:liou_control}
   \mu_p = \delta_0 \otimes\mu_0 + \Lie_{f_0}^\dagger \mu + \textstyle\sum_{k = 1}^{N_w} (f_k \cdot \nabla_x)^\dagger \sigma_k
\end{equation}

% A system with $N_d$ parameters with box uncertainty may be expressed as an instance of polytopic uncertainty with $2^{N_d}$ subsystems. Each subsystem is comprised of dynamics $\dot{x} = f_d(t,x)= f(t, x, d)$ where $d$ is fixed to a vertex of the box $\Delta = [0, 1]^{N_d}$. Since the number of subsystems (and measures) scale exponentially in $N_w$,  posing boxed uncertainty is generally more tractable than solving as a per-vertex switched system.


==> sections/discrete_lmi_brief.tex <==
\begin{rmk}
 The LMI for Discrete-Time Uncertain Peak Estimation is similar to LMI \eqref{eq:peak_lmi_un} in continuous time. If time is not included, support constraints \eqref{eq:peak_lmi_un_time}-\eqref{eq:peak_lmi_un_time2} are unnecessary. The Liouville operator $\textrm{Liou}_{\alpha \gamma}(y^0, y^p, y^k)$ is now the affine relation in moments  induced from Liouville's Equation \eqref{eq:peak_meas_un_disc_flow}  for every test function $v(x, \theta) = x^\alpha \theta^\gamma$,
 \begin{align}
 \label{eq:liou_disc_lmi_unc}
    0&= \inp{x^\alpha \theta^\gamma}{ \delta_0 \otimes \mu_0} - \inp{x^\alpha  \theta^\gamma}{\mu_p} \\
    &+ \textstyle \sum_k\inp{( f_{k}(x, \theta, w)^\alpha \theta^\gamma - x^\alpha \theta^\gamma}{\mu_k}. \nonumber
\end{align}
 \end{rmk}
%

==> sections/prelim_lmi.tex <==
 \subsection{Moment-SOS Hierarchy}
\label{sec:moment_sos}
% \urg{more citations and/or reduce content in review}
The infinite-dimensional linear measure programs \eqref{eq:peak_meas} and \eqref{eq:peak_cont} for peak estimation may be approximated through the Moment-SOS hierarchy \cite{lasserre2009moments} by a sequence of LMIs. 
% This subsection reviews topics in real semialgebraic geometry as applied to the Moment-SOS hierarchy.
% \subsubsection{Moments}
The $\alpha$-moment of a measure $\mu$ for multi-index $\alpha \in \N^n$ is $y_\alpha = \inp{x^\alpha}{\mu}$. 
The moment sequence $y$ is the infinite collection of moments $\{y_\alpha\}_{\alpha \in \N^n}$ of the measure $\mu$.
There exists a linear functional converting a polynomial $p(x)$ into a linear combination of moments:
\begin{equation}
    p(x) = \sum_{\alpha \in \N} p_\alpha x^\alpha \rightarrow \sum_{\alpha \in \N} p_\alpha y_\alpha
\end{equation}

% There exists a linear functional \urg{finish this}
% The (pseudo)-expectation of a function $p \in C(X)$ with respect to the measure $\mu$ is $\E_\mu[p] = \inp{p}{\mu}$. The operator $\E_\mu$ is an expectation only when $\mu$ is a probability measure with $\inp{1}{\mu} = y_0 = 1$. When $p$ is a polynomial, there exists a linear functional converting the (pseudo)-expectation of $p$ into a linear combination of the moments of $\mu$:
% \begin{equation}
%     \E_\mu[p] = \E_\mu\left[\sum_{\alpha \in \N} p_\alpha x^\alpha\right] = \sum_{\alpha \in \N} p_\alpha \E_\mu\left[x^\alpha\right] = \sum_{\alpha \in \N} p_\alpha y_\alpha 
% \end{equation}

The infinite set of moments $\{\inp{x^\alpha}{\mu}\}_{\alpha \in \N^n} $ uniquely specifies the measure $\mu$. Not every set of numbers $y_\alpha$ is a moment sequence for some measure $\mu$, and the problem of determining if there exists a measure $\mu$ that agrees with a set of moments $y$ such that $\inp{x^\alpha}{\mu} = y_\alpha$ is known as the Generalized Moment Problem (GMP). 
% The GMP includes the case where only a finite number of putative moments $y_\alpha$ are available. 
A measure $\mu$ whose $\alpha$-moments agree with $y_\alpha$ is known as a `representing measure' for the moment sequence $y$.
The infinite moment matrix $\M[y]$ may be defined for a moment-sequence $\{y_\alpha\}_{\alpha \in \N^n}$ as 
\begin{equation}
    \M[y]_{\alpha, \beta} = y_{\alpha+ \beta}.
\end{equation}
$\M[y]$ is a square symmetric matrix of infinite size and is indexed by monomials $(\alpha, \beta)$. If a polynomial $p=\sum_{\alpha}p_\alpha x^\alpha$ is treated as a vector $\mathbf{p}$ with coefficients $p_\alpha$, evaluation of $\inp{p(x)^2}{\mu}$ is equivalent to $\mathbf{p}^T \M[y] \mathbf{p}$. 
Nonnegativity of $\inp{p(x)^2}{\mu}$ for all $p(x)$ requires that $\M[y]$ is Positive Semidefinite (PSD). The condition  $\M[y] \succeq 0$ is necessary for the infinite sequence $y$ to represent moments of a nonnegative measure over $\R^n$.

A basic semialgebraic set $\K = \{x \mid g_i(x) \geq 0, \ i = 1, \ldots, N\}$ may be the support set for measures $\mu \in \Mp{\K}$. 
Because $\mu$ is supported over the region $\{x \mid g_1(x) \geq 0\}$, the evaluation $\inp{p(x)^2 g_1(x)}{\mu}$ is nonnegative for all polynomials $p(x) \in \R[x]$. For a polynomial $g(x) \in \R[x]$, the positive semidefinite localizing matrix associated with $g(x)$ and the moment sequence $y$ is,
\begin{equation}
    \M[g y]_{\alpha, \beta} = \sum_{\gamma \in \N^n} g_\gamma y_{\alpha+ \beta + \gamma}.
\end{equation}
The evaluation of $\inp{p(x)^2 g(x)}{\mu}$ is then equal to $\mathbf{p}^T \M[g y] \mathbf{p}$ if $y$ are the moments of a measure supported on $g(x) \geq 0$. 
When there are multiple constraints $g_i(x) \geq 0$ such as in the definition of $\K$, the following localizing matrices are all positive semidefinite:
\begin{equation}
    \forall e \in \{0, 1\}^N: \qquad \M\left[ \left(\textstyle\prod_{i=1}^N g_i^{e_i}\right) y \right] \succeq 0.
\end{equation}
When $\K$ is compact, it is sufficient for the localizing matrices $\M[g_i y]$ to be PSD $\forall i = 1, \ldots, N$


The moment matrix $\M[y]$ and localizing matrices $\M[g_i y]$ are infinite-dimensional. A degree-$r$ finite truncation of these matrices keeps moments up to order $2r$, which are located in the upper-left corners of the infinite dimensional matrices. The truncated moment matrix $\M_r[y]$ has size $\binom{n+r}{r}$ corresponding to the monomials of $x$ with degree $\leq k$. The localizing matrix $\M_{k - \textrm{deg}(g_i)}[g_i y]$ has size $\binom{n+r - \textrm{deg}(g_i)}{r-\textrm{deg}(g_i)}$, and similarly involves moments up to order $2r$. 




==> sections/prelim_occupation.tex <==
\subsection{Occupation Measures}

% Review occupation measures (initial, occupation). Include marginalization over $w$

% An occupation measure 


A trajectory of the dynamical system $\dot{x}=f(t,x)$ for times $t \in [0, T]$ starting at an initial condition $x_0 \in X_0$ may be denoted as $x(t \mid x_0)$ . Let $\mu_0 \in \Mp{X_0}$ be a measure distributed over initial conditions. The average occupation measure with respect to $\mu_0$ returns the expected amount of time that trajectories spend in a particular time-space region $A \subseteq [0, T], \ B  \subseteq X$ \cite{lewis1980relaxation},
\begin{equation}
    \label{eq:occ_measure}
    \mu(A \times B) = \int_{[0, T] \times X_0} I_{A \times B}((t, x(t \mid x_0))) d \mu_0(x_0) dt.
\end{equation}
The measure $\mu$ satisfies $\mu([0, T] \times X) = T$. The terminal measure $\mu^T$ that follows trajectories until time $T$ is:
\begin{equation}
    \label{eq:occ_terminal}
    \mu^T(B) = \int_{X_0} I_{B}((x(T \mid x_0)) d \mu_0(x_0).
\end{equation}
% Assuming that trajectories spend all time $[0, T]$ in $X$, then $\mu([0, T] \times X) = T$.
% \urg{Is a terminal measure necessary? We can go straight to the peak with liouville}. 
For a test function $v(t, x) \in C^1([0, T], \times X)$, the Lie derivative of $v$ with respect to the vector field $f$ is:
\begin{equation}
    \label{eq:lie_deriavite}
    \Lie_f v(t,x) = \partial_t v(t, x)+ \nabla_x v(t,x) \cdot f(t, x).
\end{equation}
The three measures $\mu_0, \mu_T, \mu$ are related by Liouville's equation for all test functions $v(t, x) \in C^1([0, T], \times X)$:
\begin{align}
\inp{v(T, x)}{\mu_T} &= \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t,x)}{\mu}. \label{eq:liou_int}
\end{align}
Equation \eqref{eq:liou_int} may be expressed in a weak sense by,
\begin{align}
\delta_T \otimes \mu_T &= \delta_0 \otimes \mu_0 + \Lie_f^\dagger \mu. \label{eq:liou_mom}
\end{align}
Equation \eqref{eq:liou_mom} is an equivalent statement for Liouville's equation where the adjoint $\inp{\Lie_f v}{\mu} = \inp{v}{\Lie^\dagger_f \mu}$. Moments of $\mu$  can be computed by evaluating $\inp{v(t,x)}{\mu}$ where the test function $v$ is a monomial.  Equation \eqref{eq:liou_mom} is an infinite set of linear constraints in terms of moments of $\mu_0, \mu_T, \mu$.

External controls or disturbances can be added into an occupation measure framework. For an input $w(t) \in W$ and a subset $D \subseteq W$, the disturbance-occupation measure $\mu^w$ is:
\begin{align}
    \label{eq:occ_measure_d}
    &\mu^w(A \times B \times D) = \\
    &\quad \int_{[0, T] \times X_0} I_{A \times B \times D}((t, x(t), w(t)) \mid x_0) d \mu_0(x_0) dt. \nonumber
\end{align}
The disturbance $w(t)$ may be relaxed into a distribution $\xi(w \mid x, t)$ known as a Young Measure \cite{young1942generalized, lewis1980relaxation}.
Liouville's equation with a relaxed disturbance $\xi(w \mid x, t)$ influencing dynamics $f(t, x, w)$ for all $v(t, x) \in C^1([0, T]\times X)$ is,
\begin{align}
\label{eq:liou_d}
\inp{v(T, x)}{\mu_T} &= \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t, x)}{\mu^w}. \end{align}
Equivalent expressions are formed by rearranging operators,
\begin{align}
\inp{v}{\delta_T \otimes \mu_T} &= \inp{v}{\delta_0 \otimes \mu_0} + \inp{\Lie_f v}{\mu^w} & \forall v \\
\inp{v}{\delta_T \otimes \mu_T} &= \inp{v}{\delta_0 \otimes \mu_0} + \inp{v}{\Lie_f^\dagger \mu^w} & \forall v \label{eq:weak_before_sum}\\
\inp{v}{\delta_T \otimes \mu_T} &= \inp{v}{\delta_0 \otimes \mu_0 + \pi^{tx}_\#\Lie_f^\dagger \mu^w} & \forall v.\label{eq:weak_after_sum}
\end{align}

The measures of the two summands on the right hand side of \eqref{eq:weak_before_sum} reside in different spaces, as $\delta_0 \otimes \mu_0 \in \Mp{[0, T] \times X}$ while $\Lie_f^\dagger \mu^w \in \Mp{[0, T] \times X \times W}$. The $(t,x)$-marginalization $\pi^{tx}_\# \Lie^\dagger_f \mu^w \in \Mp{[0, T] \times X}$ allows the measures to be added together inside the duality pairing in \eqref{eq:weak_after_sum}. The duality pairings $\inp{v(t,x)}{\Lie^\dagger_f \mu^w}$ and $\inp{v(t,x)}{\pi^{tx}_\#\Lie^\dagger_f \mu^w}$ are equal for all $v \in C^1([0, T] \times X)$
because $v(t,x)$ is not a function of $w$. The weak disturbed Liouville's Equation is derived from \eqref{eq:weak_after_sum}  by treating  $\forall v(t, x) \in C^1([0, T]\times X)$ as implicit,
\begin{equation}
    \delta_T \otimes \mu_T = \delta_0 \otimes \mu_0 + \pi^{tx}_\# \Lie^\dagger_f \mu^w.
\end{equation}



% The Lie term  in \eqref{eq:liou_d} marginalizes out the relaxed disturbance $\xi$, and can be written as $\inp{\Lie_f v(t, x)}{\mu^w} = \inp{v(t, x)}{\pi^{tx}_\# \Lie^\dagger_f \mu^w}$ with projection map $\pi^{t x}: [0, T] \times X \times W \rightarrow [0, T] \times X$.


% The weak formulation of \eqref{eq:liou_d} holding for all test functions $v(t, x) \in C([0, T]\times X)$ is,
% The weak formulation of \eqref{eq:liou_d} may be written by using the pushforward of the projection map $\pi^{t x}: [0, T] \times X \times W \rightarrow [0, T] \times X$ in order to marginalize out the relaxed disturbance,

% \begin{equation}
% \label{eq:liou_d}
% \delta_T \otimes \mu_T = \delta_0 \otimes \mu_0 + \pi^{tx}_\#\Lie_f^\dagger \mu^d
% \end{equation}
% The projection operator $\pi^{tx}_\#$ marginalizes the input $d(t)$ from the distribution $\xi$ of possible disturbances. 
% The measure $\mu^d$ is known  as a Young Measure, and acts as a relaxed disturbance or control  \urg{is this correct?}.

% There exists a $\mu^d$ which solves Equation \eqref{eq:liou_int} such that the support of $\mu^d$ is contained on the graph $(t, x(t), d(t))$ \cite{lasserre2008nonlinear}.

% control-occupation measure $\mu^w$ is supported on the graph

% by introducing a measure $\mu^w$:



% Write about the control-occupation measure.


==> sections/prelim_peak.tex <==
\subsection{Peak Estimation}
\label{sec:peak}
% The peak estimation problem aims to solve:
% The peak estimation problem in \cite{miller2020peak} solves \eqref{eq:peak_traj} without the presence of a disturbance $w$.

Peak estimation programs without uncertainty in a compact space $X \subset \R^n$ may be upper bounded as infinite-dimensional LPs in occupation measures \cite{cho2002linear}, 
% These infinite dimensional programs have been approximated by discretizing the state space into finite-dimensional LPs \cite{cho2002linear}, or by using the Moment-SOS hierarchy with a set of LMIs in combinatorially increasing size \cite{fantuzzi2020bounding}. 
% It is assumed that the state sets $X$ and $X_0$ are compact basic semialgebraic sets \cite{lasserre2009moments} to assure convergence in increasing degree of the Moment-SOS hierarchy to an accumulation point.
% The measure program for peak estimation from \cite{cho2002linear} is,
\begin{subequations}
\label{eq:peak_meas}
\begin{align}
p^* = & \ \textrm{max} \quad \inp{p(x)}{\mu_p} \label{eq:peak_meas_obj} \\
    & \mu_p = \delta_0 \otimes\mu_0 + \Lie_f^\dagger \mu \label{eq:peak_meas_flow}\\
    & \mu_0(X) = 1 \label{eq:peak_meas_prob}\\
    & \mu, \mu_p \in \Mp{[0, T] \times X} \label{eq:peak_meas_peak}\\
    & \mu_0 \in \Mp{X_0}. \label{eq:peak_meas_init}
\end{align}
\end{subequations}
The peak probability measure $\mu_p$ is a free-time terminal measure with a similar form to \eqref{eq:occ_terminal}, where the time-stopping can occur anywhere between $t \in [0, T]$ in order to extremize $p(x)$.
The occupation measure $\mu$ connects $\mu_0$ and $\mu_p$ by Liouville's equation \eqref{eq:peak_meas_flow}, and one consequence is that $\inp{1}{\mu} = \inp{t}{\mu_p}$ with $v(t,x) = t$. 
The dual problem to the measure program \eqref{eq:peak_meas} is posed over continuous functions, 
\begin{subequations}
\label{eq:peak_cont}
\begin{align}
    d^* = & \ \min_{\gamma \in \R} \quad \gamma & \\
    & \forall x \in X_0: \nonumber \\
    & \quad {\gamma} \geq {v(0, x)}   \label{eq:peak_cont_init}\\
    & \forall (t, x) \in [0, T] \times X: \nonumber \\
    & \quad \Lie_f v(t, x) \leq 0 \label{eq:peak_cont_f}\\
    & \quad v(t, x) \geq p(x)  \label{eq:peak_cont_p} \\
    &v(t, x) \in C^1([0, T]\times X). \label{eq:peak_cont_v}
\end{align}
\end{subequations}
% \begin{subequations}
% \label{eq:peak_cont}
% \begin{align}
%     d^* = & \ \min_{\gamma \in \R} \quad \gamma & \\
%     & {\gamma} \geq {v(0, x)}  &  \forall x \in X_0 \label{eq:peak_cont_init}\\
%     & \Lie_f v(t, x) \leq 0 & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_f}\\
%     & v(t, x) \geq p(x) & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_p} \\
%     &v \in C^1([0, T]\times X) \label{eq:peak_cont_v}&
% \end{align}
% \end{subequations}
% $v(t,x)$ is referred to as an auxiliary function in \cite{fantuzzi2020bounding}, and is an upper bound on the cost function $p(x)$ by \eqref{eq:peak_cont_p}. 
For computational purposes, it is assumed that the set $[0, T] \times X$ is compact. This compactness asssures that programs \eqref{eq:peak_meas} and \eqref{eq:peak_cont} satisfy strong duality, since all measures have bounded moments and the image of the affine map in \eqref{eq:peak_meas_flow}-\eqref{eq:peak_meas_init} is closed and bounded (Theorem C.20 of \cite{lasserre2009moments}). These programs form an upper bound $p^* = d^* \geq P^*$ on \eqref{eq:peak_traj} without $(\theta, w)$, which is tight to $p^* = P^*$ with the assumption that $[0, T] \times X$ is compact (Sec. 2.3 of \cite{fantuzzi2020bounding} and \cite{lewis1980relaxation}).
% This upper bound will be tight with $p^*=d^*=P^*$ if the auxiliary function $v(t, x)$ in \eqref{eq:peak_cont_v} is allowed to be discontinuous \cite{fantuzzi2020bounding}. 
% $v(t,x)$ is an upper bound on the on the cost function $p(x)$ by \eqref{eq:peak_cont_p} for all time $t \in [0, T]$, and 
The sublevel set $\{(t,x) \mid v(t,x) \leq \gamma\}$ is an invariant set containing the graph of all trajectories starting from $X_0$ in time $[0, T]$.

% \urg{Talk about moment relaxations? SOS, polynomials?}

Problems \eqref{eq:peak_meas} and \eqref{eq:peak_cont} are a pair of infinite-dimensional linear programs. The work in \cite{cho2002linear} approximates these problems by a discretized linear program over a fine mesh. The method in \cite{fantuzzi2020bounding} bounds \eqref{eq:peak_cont} with a sum-of-squares (SOS) relaxation of polynomial nonnegativity constraints. The SOS relaxation produces a converging sequence of upper bounds to $d^*$ when $[0, T] \times X$ is compact. This SOS formulation is dual to LMIs in moments of occupation measures formed by a finite truncation of \eqref{eq:peak_meas} \cite{lasserre2009moments}. 
The degree-$d$ moment matrix for $\mu_p$ defined over the $1+N_x $ variables $(t, x)$ is a symmetric PSD matrix of size $\binom{1+N_x+d}{d}$. 
Near-optimal trajectories extremizing $p(x)$ may be recovered from LMI solutions if the moment matrices obey rank conditions \cite{miller2020recovery}. These trajectories may also be localized by sublevel sets of the dual $v(t,x)$ following the method in \cite{fantuzzi2020bounding}.
% The sequence of optima 
% Optimal trajectories extremizing $p(x)$ may be approximately recovered from LMI solutions if the moment matrices obey rank conditions \cite{miller2020recovery}.

% \urg{If space permits, put in more content about LMIs and write the LMI for the unified uncertain peak problem.}

% A degree-$\delta$ LMI relaxation of \eqref{eq:peak_meas} or SOS relaxation of \eqref{eq:peak_cont} generically results in  

% In an LMI relaxation, the coefficients of the degree-$2d$ polynomial $v(t,x)$ can be recovered from dual variables of the truncated degree-$d$ Moment program.


% \subsection{Peak Estimation}


==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Notation}
% Either a table or written out sections.
Let $\R^n$ be an $n$-dimensional real Euclidean space, and $\R[x]$ be the set of polynomials in $x$ with real-valued coefficients. For a space $X \subseteq \R^n$, the sets $C(X)$ and $C_+(X)$ are respectively the set of continuous functions on $X$ and its nonnegative subcone. The subcone $C^1(X) \subset C(X)$ is composed of continuous functions with continuous first derivatives. $\Mp{X}$ is the set of nonnegative Borel measures over $X$, and a duality pairing exists $\inp{f}{\mu} = \int_X f(x) d \mu(x)$ for all $f \in C(X), \ \mu \in \Mp{X}$. For every linear operator $\Lie$, there exists a unique linear adjoint $\Lie^\dagger$ such that $\inp{\Lie f}{\mu} = \inp{f}{\Lie^\dagger \mu}, \ \forall f,\mu$ is satisfied. An indicator function is $I_A(x)=1$ for a subset $A \subseteq X$ if $x \in A$ and $I_A(x) = 0$ otherwise. The measure of a set $A$ with respect to $\mu$ is $\mu(A) = \int_X I_A(x) d\mu$. The quantity $\mu(X) = \inp{1}{\mu}$ is known as the `mass', and $\mu$ is a probability measure if $\mu(X) = 1$. The Dirac delta $\delta_x \in \Mp{X}$ is a probability measure supported only on $x$. For measures $\mu \in \Mp{X}, \ \nu \in \Mp{Y}$, the product measure satisfies $(\mu \otimes \nu)(A \times B) = \mu(A)\nu(B)$ for all $A \in X, \ B \in Y$. The projection map $\pi^x: X \times Y \rightarrow X$ returns only the $x$ coordinate $(x, y) \rightarrow x$. The pushforward operator $\#$ on measures satisfies $\inp{v(x)}{f_\# \mu} = \inp{v(f(x))}{\mu}$ for any test function $v \in C(X)$ and function $f$. 

% This may be coupled with the projection operator: $\inp{v(\pi^x (x,y))}{\mu} = \inp{v(x)}{\mu}$ 


% The projection $\pi_{x} \eta$ of a measure $\eta \in \Mp{X \times Y}$ satisfies $\pi_x \eta(A \times B) = \eta(A)$

% Define $\R^n, \ \R[x], \ \R[x]_{\leq d}, \ C(X), \ C_+(X), \ \Mp{X}$, $\inp{f}{\mu} = \int_X{f d \mu}, \ \mu(X), \mu_1 \otimes \mu_2, \pi_t \mu$
% \urg{Fill this out}

% \subsection{Uncertainty Models}

% Dynamics are $\dot{x} = f(t, x, w)$. Uncertainty $w$ is in a set $W \subset \R^{N_w}$ for all time $t$. In numerical computation, $W$ must be compact.

% Time-independent uncertainty: $\partial_t w = 0$ and $w$ are constant throughout trajectories.

% Time-varying uncertainty: $w$ can change arbitrarily in time in the valid region $W$. No assumptions of continuity. Specific applications may add additional constraints on moments of the noise process $w$, such as $\norm{w}_2^2 = \int_{0}^T \norm{w(t)}^2_2 d t \leq 1$.

% Affine uncertainty: A specific form of time-varying dynamics which are $\dot{x} = f(t,x) + g(t,x) w$. This affine structure may make computation easier. Specific forms include polytopic (switching) uncertainty with $w \geq 0$ and $\sum_i w = 1$, and box uncertainty where $w_i \in [0, \bar{w}_i]$.

\subsection{Occupation Measures}

% Review occupation measures (initial, occupation). Include marginalization over $w$

% An occupation measure 


A trajectory of the dynamical system $\dot{x}=f(t,x)$ starting at an initial condition $x_0 \in X_0$ may be represented as $x(t \mid x_0)$ for times $t \in [0, T]$. Let $\mu_0 \in \Mp{X_0}$ be a measure distributed over initial conditions. The average occupation measure with respect to $\mu_0$ returns the expected amount of time that trajectories spend in a particular time-space region $A \subseteq [0, T], \ B  \subseteq X$ \cite{lewis1980relaxation},

\begin{equation}
    \label{eq:occ_measure}
    \mu(A \times B) = \int_{[0, T] \times X_0} I_{A \times B}((t, x(t \mid x_0)) d \mu_0(x_0) dt.
\end{equation}

The measure $\mu$ satisfies $\mu([0, T] \times X) = T$. The terminal measure $\mu^T$ that follows trajectories until time $T$ is:

\begin{equation}
    \label{eq:occ_terminal}
    \mu^T(B) = \int_{X_0} I_{B}((x(T \mid x_0)) d \mu_0(x_0).
\end{equation}

% Assuming that trajectories spend all time $[0, T]$ in $X$, then $\mu([0, T] \times X) = T$.

% \urg{Is a terminal measure necessary? We can go straight to the peak with liouville}. 
For a test function $v(t, x) \in C^1([0, T], \times X)$, the Lie derivative of $v$ with respect to the vector field $f$ is:
\begin{equation}
    \label{eq:lie_deriavite}
    \Lie_f v(t,x) = \partial_t v(t, x)+ \nabla_x v(t,x)^T f(t, x).
\end{equation}
The three measures $\mu_0, \mu, \mu_T$ are related by Liouville's equation for all test functions $v(t, x) \in C^1([0, T], \times X)$:
\begin{align}
\inp{v(T, x)}{\mu_T} &= \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t,x)}{\mu} \label{eq:liou_int}
\end{align}
Equation \eqref{eq:liou_int} may be equivalently expressed in a weak sense by,
\begin{align}
\delta_T \otimes \mu_T &= \delta_0 \otimes \mu_0 + \Lie_f^\dagger \mu \label{eq:liou_mom}
\end{align}
Equation \eqref{eq:liou_mom} is an equivalent statement for Liouville's equation where the adjoint $\inp{\Lie_f v}{\mu} = \inp{v}{\Lie^\dagger_f \mu}$. Moments of $\mu$  can be computed by evaluating $\inp{v(t,x)}{\mu}$ where the test function $v$ is a monomial.  Equation \eqref{eq:liou_mom} is an infinite set of linear constraints in terms of moments of $\mu_0, \mu, \mu_T$.

External controls or disturbances can be added into an occupation measure framework. For an input $d(t) \in \Delta$ and a subset $D \subseteq \Delta$, the disturbance-occupation measure $\mu^d$ is:
\begin{align}
    \label{eq:occ_measure_d}
    &\mu^d(A \times B \times D) = \\
    &\quad \int_{[0, T] \times X_0} I_{A \times B \times D}((t, x(t), d(t)) \mid x_0) d \mu_0(x_0) dt. \nonumber
\end{align}
The disturbance $d(t)$ may be relaxed into a distribution $\xi(d \mid x, t)$ known as a Young Measure \cite{young1942generalized, lewis1980relaxation}.
The Liouville Equation with a relaxed disturbance $\xi$ is,
\begin{equation}
\label{eq:liou_d}
\inp{v(T, x)}{\mu_T} = \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t, x)}{\mu^d}
\end{equation}.
% \begin{equation}
% \label{eq:liou_d}
% \delta_T \otimes \mu_T = \delta_0 \otimes \mu_0 + \pi^{tx}_\#\Lie_f^\dagger \mu^d
% \end{equation}
% The projection operator $\pi^{tx}_\#$ marginalizes the input $d(t)$ from the distribution $\xi$ of possible disturbances. 
% The measure $\mu^d$ is known  as a Young Measure, and acts as a relaxed disturbance or control  \urg{is this correct?}.

% There exists a $\mu^d$ which solves Equation \eqref{eq:liou_int} such that the support of $\mu^d$ is contained on the graph $(t, x(t), d(t))$ \cite{lasserre2008nonlinear}.

% control-occupation measure $\mu^w$ is supported on the graph

% by introducing a measure $\mu^w$:



% Write about the control-occupation measure.

\subsection{Peak Estimation}
\label{sec:peak}
% The peak estimation problem aims to solve:
% The peak estimation problem in \cite{miller2020peak} solves \eqref{eq:peak_traj} without the presence of a disturbance $w$.

Peak estimation programs may be upper bounded as infinite-dimensional linear programs (LPs) in occupation measures. These infinite dimensional programs have been approximated by discretizing the state space into finite-dimensional LPs \cite{cho2002linear}, or by using the Moment-SOS hierarchy with a set of LMIs in combinatorially increasing size \cite{fantuzzi2020bounding}. 



% It is assumed that the state sets $X$ and $X_0$ are compact basic semialgebraic sets \cite{lasserre2009moments} to assure convergence in increasing degree of the Moment-SOS hierarchy to an accumulation point.

The measure program for peak estimation from \cite{cho2002linear} is,

\begin{subequations}
\label{eq:peak_meas}
\begin{align}
p^* = & \ \textrm{max} \quad \inp{p(x)}{\mu_p} \label{eq:peak_meas_obj} \\
    & \mu_p = \delta_0 \otimes\mu_0 + \Lie_f^\dagger \mu \label{eq:peak_meas_flow}\\
    & \mu_0(X) = 1 \label{eq:peak_meas_prob}\\
    & \mu, \mu_p \in \Mp{[0, T] \times X} \label{eq:peak_meas_peak}\\
    & \mu_0 \in \Mp{X_0}. \label{eq:peak_meas_init}
\end{align}
\end{subequations}
The peak probability measure $\mu_p$ is a free-time terminal measure with a similar form to \eqref{eq:occ_terminal}, where the time-stopping can occur anywhere between $t \in [0, T]$ in order to extremize $p(x)$.
The occupation measure $\mu$ connects $\mu_0$ and $\mu_p$ by Liouville's equation \eqref{eq:peak_meas_flow}, and one consequence is that $\inp{1}{\mu} = \inp{t}{\mu_p}$. 
The dual problem to the measure program \eqref{eq:peak_meas} is posed over continuous functions, 
\begin{subequations}
\label{eq:peak_cont}
\begin{align}
    d^* = & \ \min_{\gamma \in \R} \quad \gamma & \\
    & {\gamma} \geq {v(0, x)}  &  \forall x \in X_0 \label{eq:peak_cont_init}\\
    & \Lie_f v(t, x) \leq 0 & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_f}\\
    & v(t, x) \geq p(x) & \forall (t, x) \in [0, T] \times X \label{eq:peak_cont_p} \\
    &v \in C^1([0, T]\times X) \label{eq:peak_cont_v}&
\end{align}
\end{subequations}

% $v(t,x)$ is referred to as an auxiliary function in \cite{fantuzzi2020bounding}, and is an upper bound on the cost function $p(x)$ by \eqref{eq:peak_cont_p}. 

For computational purposes, it is assumed that the set $[0, T] \times X$ is compact. This compactness asssures that programs \eqref{eq:peak_meas} and \eqref{eq:peak_cont} satisfy strong duality, since all measures have bounded moments and the image of the affine map in \eqref{eq:peak_meas_flow}-\eqref{eq:peak_meas_init} is closed and bounded (Theorem C.20 of \cite{lasserre2009moments}). These programs form an upper bound $p^* = d^* \geq P^*$ on \eqref{eq:peak_traj} without $(w, d)$. This upper bound will be tight with $p^*=d^*=P^*$ if the auxiliary function $v(t, x)$ in \eqref{eq:peak_cont_v} is allowed to be discontinuous \cite{fantuzzi2020bounding}. 
% $v(t,x)$ is an upper bound on the on the cost function $p(x)$ by \eqref{eq:peak_cont_p} for all time $t \in [0, T]$, and 
The sublevel set $\{(t,x) \mid v(t,x) \leq \gamma\}$ is an invariant set containing the graph of all trajectories starting from $X_0$ in time $[0, T]$.

% \urg{Talk about moment relaxations? SOS, polynomials?}

Problems \eqref{eq:peak_meas} and \eqref{eq:peak_cont} are a pair of infinite-dimensional linear programs. The work in \cite{cho2002linear} approximates these problems by a discretized linear program over a fine mesh. \cite{fantuzzi2020bounding} bounds \eqref{eq:peak_cont} with a sum-of-squares (SOS) relaxation of polynomial nonnegativity constraints. The SOS relaxation produces a converging sequence of upper bounds to $d^*$ when $[0, T] \times X$ is compact. This SOS formulation is dual to LMIs in moments of occupation measures formed by a finite truncation of \eqref{eq:peak_meas} \cite{lasserre2009moments}, where the size of the PSD matrix variables rises combinatorially with degree. 
% SOS and LMI relaxations produce Semidefinte Programs where the size of the PSD matrix variables rise combinatorially with degree. 
The degree-$\delta$ moment matrix for $\mu_p$ defined over the $1+N_x $ variables $(t, x)$ is a symmetric PSD matrix of size $\binom{1+N_x+\delta}{\delta}$. The sequence of optima 
Optimal trajectories extremizing $p(x)$ may be approximately recovered from LMI solutions if the moment matrices obey rank conditions \cite{miller2020recovery}.

% \urg{If space permits, put in more content about LMIs and write the LMI for the unified uncertain peak problem.}

% A degree-$\delta$ LMI relaxation of \eqref{eq:peak_meas} or SOS relaxation of \eqref{eq:peak_cont} generically results in  

% In an LMI relaxation, the coefficients of the degree-$2d$ polynomial $v(t,x)$ can be recovered from dual variables of the truncated degree-$d$ Moment program.


% \subsection{Peak Estimation}

%  Summarize peak estimation paper formulation

==> sections/summary.tex <==
This paper has the following structure: Section \ref{sec:preliminaries} reviews preliminaries such as occupation measures and peak estimation. Section \ref{sec:uncertainty} presents uncertainty models, and a unified uncertain peak estimation model is presented in Section \ref{sec:unified}. Section \ref{sec:discrete} extends uncertain peak estimation to discrete systems. 
% Efficacy is demonstrated in section \ref{sec:examples}, and t
The paper is concluded in Section \ref{sec:conclusion}.

==> sections/switching.tex <==
\subsection{Switching Uncertainty}

\label{sec:affine}

Many dynamical systems exhibit an affine structure in terms of the disturbance $d \in \Delta$:
\begin{equation}
\label{eq:affine_base}
    \dot{x} = f(t,x,d) = f_0(t,x,d) + \sum_{k=1}^{N_d} d_k(t) f_k(t,x,d)
\end{equation}
% Peak estimation of input-affine systems with time-varying uncertainty may proceed through the methods of Problem \eqref{eq:peak_meas_w} and \eqref{eq:peak_cont_w}. 
% In some specific cases the affine structure may be used to simplify computation
% \cite{majumdar2014convex, korda2014controller}.
% \subsubsection{Polytopic Uncertainty}
% \label{sec:polytopic}

Polytopic uncertainty is an instance of time-varying uncertainty where all $d_i(t) \geq 0$ and $\sum_i d_i(t) = 1$. The dynamics from \eqref{eq:affine_base} may be divided into:
\begin{equation}
\label{sec:poly_split}
    \sum_{k=1}^{N_d} d_k(t) (f_0(t,x,d) + f_k(t,x,d) ) = \sum_{w=1}^{N_w} d_k(t) \tilde{f}_k(t,x,d)
\end{equation}
for merged dynamics $\tilde{f}_k(t,x,w)$ on each parameter $w_k$. Dynamics in $f$ are convex combinations of $\tilde{f}_k(t,x,d)$. Mixed dynamics may be realized as a system switching arbitrarily quickly between base dynamics $\tilde{f}_k(t,x,d)$. The occupation measure $\mu \in \Mp{[0, T]\times X}$ and adjoint Lie derivative of constraint \eqref{eq:peak_meas_flow} can be decomposed \cite{henrion2012measures},
\begin{equation}
\label{eq:occ_poly}
    \mu = \textstyle\sum_k \mu_k \qquad \Lie^\dagger \mu = \textstyle\sum_k \Lie^\dagger_{\tilde{f}_k} \mu_k
\end{equation}
A valid auxiliary function $v(t,x)$ from \eqref{eq:peak_cont_f} must decrease along all subsystems \cite{parrilo2008approximation, vlassis2014polytopic}.
\begin{equation}
    \Lie_{\tilde{f}_k} v(t, x) \leq 0 \quad \forall (t, x) \in [0, T] \times X, \ k=1\ldots N_d \label{eq:peak_cont_f_poly}
\end{equation}
The moments $\inp{1}{\mu_k}$ are the expected amount of time that trajectories spend following dynamics $\tilde{f}_k$. 


\label{sec:switching}
Switching uncertainty is a generalization of polytopic uncertainty.
Let $\{X^k\}_{k=1}^{N_s}$ be a closed cover of $X$ for $k=1\ldots N_s$, which is a set of not necessarily disjoint closed subsets $X^k \subseteq X$ such that $\cup_k X^k = X$. Further, let $\dot{x} = \tilde{f}_k(t,x)$ be dynamics that evolve on each $X_k$. 
The closed cover formalism generalizes partitions of $X$ where $X^k \cap X^{k'} = \varnothing \ \forall k \neq k'$ and arbitrary switching where $X^k = X \ \forall k$. The switched measure program introduces an occupation measure $\mu_k \in \Mp{[0, T] \times X^k}$ for each subsystem $\tilde{f}_k$ subject to \eqref{eq:occ_poly}. The nonnegativity condition \eqref{eq:peak_cont_f_poly} in $v(t,x)$ is restricted to each region $[0, T] \times X_k$
\begin{equation}
    \Lie_{\tilde{f}_k} v(t, x) \leq 0 \quad \forall (t, x) \in [0, T] \times X_k, \ k=1\ldots N_d \label{eq:peak_cont_f_switch}
\end{equation}

% \subsubsection{Box Uncertainty}
% \label{sec:box}
% % All parameters are in a box

% Box uncertainty is a case where the region $\Delta$ is a box, and there are no other constraints on $d(t)$. With a proper scaling of dynamics, all $d$ can be constrained to the region $d_k(t) \in [0,1]$. The methods in \cite{korda2014controller, majumdar2014convex} introduce box-measures $\{\sigma_k \in \Mp{[0,T] \times X} \}_{k=1}^{N_d}$ such that for all subsets $A \times B \in [0, T] \times X$.
% \begin{equation}
%     \int_{A\times B} d_k(t) d \mu = \int_{A \times B} d \sigma
% \end{equation}

% Each measure $\sigma_k$ is absolutely continuous with respect to the occupation measure $\mu$ $(\sigma(A \times B) \leq \mu(A \times B), \ \forall A \in [0, T], \ \forall B \in X$. It therefore holds that there exists a nonnegative measure $\hat{\sigma}_k \in \Mp{[0, T] \times X}$ such that $\sigma_k + \hat{\sigma}_k = \mu$ for each $k$.

% % By the Jordan decomposition there exists nonnegative complement measures $\hat{\sigma}_k \in \Mp{[0,T] \times X}$ such that $\sigma_k + \hat{\sigma}_k = \mu$ for each $k = 1, \ldots, N_d$. 

% The Liouville equation \eqref{eq:liou_d} may be expressed in terms of $\sigma$ for all test functions $v (t, x) \in C^1([0, T] \times X)$ as
% \begin{equation}
%     \inp{v(t, x)} {\mu_p} = \inp{v(0, x)}{\mu_0} + \inp{\Lie_{f_0}  v(t, x)}{\mu} + + \textstyle\sum_{k = 1}^{N_w} \inp{f_k \cdot \nabla_x v (t,x)}{ \sigma_k}
% \end{equation}
% \begin{equation}
% \label{eq:liou_control}
%   \mu_p = \delta_0 \otimes\mu_0 + \Lie_{f_0}^\dagger \mu + \textstyle\sum_{k = 1}^{N_w} (f_k \cdot \nabla_x)^\dagger \sigma_k
% \end{equation}




==> sections_arxiv_additional/conclusion.tex <==
\section{Conclusion}

\label{sec:conclusion}

% \urg{Conclude the paper. Summarize the problem and important findings. Add some extensions and future work.}

The problem of peak estimation with uncertainty may be upper bounded with an infinite-dimensional LP in occupation measures, and approximated by a sequence of LMIs. Time-independent and time-dependent (including box, and switching) uncertainties  are incorporated into this measure framework for continuous and discrete systems. Specific application of this method towards the analysis of linear systems was discussed. Future work includes performing peak estimation with further specialized uncertainty structures.

==> sections_arxiv_additional/extensions.tex <==
\section{Extensions}
% \urg{Should this be included at all, or left for arxiv? pushing the 6-page limit}
\label{sec:extensions}

This section briefly covers possible extensions of the uncertain peak estimation method. These extensions are all compatible with each other, and can be combined if desired.




\subsection{Running and State Costs}
Section 5 of \cite{fantuzzi2020bounding} proposes a method to penalize a running cost as well as a state cost in peak estimation. If $J(t, x)$ is a running cost of a continuous-time system with (possibly time-varying) state cost $p(t, x)$, the augmented objective of problem \eqref{eq:peak_traj} would be,
\begin{equation}
    \min p(t, x) + \int_{t' = 0}^t {J(t', x(t \mid x_0, w, d(t')) dt'}
\end{equation}
The discrete-time augmented objective for a system with costs $(p(x), J(x))$ is,
\begin{equation}
    \min p(x) + \sum_{t' = 0}^t {J(x(t \mid x_0, w, d_{t'}) }
\end{equation}
The weak formulations in problem \eqref{eq:peak_meas_un} or \eqref{eq:peak_meas_un_disc} would then have an objective,
\begin{equation}
    \min \inp{p}{\mu_p} + \inp{J}{\mu}
\end{equation}



For a switched system with $N_s$ states, each state may optionally have a state cost $p_k(t, x)$ and possess a running cost $J_k(t, x)$. Each running cost $J_k(t, x)$ only accrues during times $t$ when the trajectory $x(t \mid x_0, w, d(t))$ is following dynamics $f_k$ inside region $X_k$. To handle this per-state costs, the peak measure $\mu_p$ may be split into switch-peak measures $\mu_{pk} \in \Mp{[0, T] \times X_k \times W}$ such that $\mu_{p} = \sum_k \mu_{pk}$. The weak-formulation objectives \eqref{eq:peak_meas_un_obj} or \eqref{eq:peak_meas_un_disc_obj} may then be replaced with,
\begin{equation}
    \textrm{max} \quad \sum_{k=1}^{N_s} \inp{p_{k}(t,x)}{\mu_{pk}} + \inp{J_k(t, x)}{\mu_k} \label{eq:compound_objective}
\end{equation}

Constraint \eqref{eq:peak_cont_un_flow} would have a $J_k$ term, 
\begin{align}&\forall (t, x, w, d) \in [0, T] \times X_k \times W \times \Delta: \quad \forall k \\
    & \qquad \Lie_{f_{0k}} v(t, x, w) + \textstyle \sum_{\ell} \zeta_{k \ell}(t, x, w, d) + J_k(t, x) \leq 0 \label{eq:peak_cont_un_flow_J}.
\end{align}
and constraint \eqref{eq:peak_cont_un_p} would be replaced with a $p_k$ term,
\begin{align}&\forall (t, x, w) \in [0, T] \times X_k \times W : \quad \forall k \\
    & \qquad v(t, x, w) \geq p_k(x) \label{eq:peak_cont_un_flow_p}.
\end{align}


Similarly, constraint \eqref{eq:peak_cont_disc_flow} for a  discrete system in would have a $J_k$ term,
\begin{align}
        & \forall (x, w, d) \in  X_k \times W \times \Delta: \quad \forall k \nonumber \\
    & \quad v(f_k(x), w) -v(x, w) + J_k(x)  \leq  \alpha
\end{align}
and constraint \eqref{eq:peak_cont_disc_p} is replaced by a $p_k$ term, 
\begin{align}&\forall (x, w) \in X_k \times W : \quad \forall k \\
    & \qquad v(x, w) \geq p_k(x) \label{eq:peak_cont_un_p_J}.
\end{align}




\subsection{Integral Constraints}
\urg{I would need to rewrite my sampler to do the integral constraints and/or fixed noise processes.}

% \subsection{Disturbance Characterization}
Properties of the disturbance $d(t)$ may be specified by moment constraints on the disturbance-occupation measure $\mu^d$ defined in \eqref{eq:occ_measure_d}.

For any polynomial $h(d) \in \R[d]$, the integral quantity $\int_{t=0}^T h(d(t)) dt$ may be reformulated as $\inp{h(d)}{\mu^d}$.
% As an example, the process $d(t)$ may be constrained to have unit $L_2$ norm by imposing that $ \inp{\norm{d}_2^2}{\mu} = 1$.
As an example, the $L_2$-norm of the process $d(t)$ along system trajectories is $\norm{d(t)}_2 = \sqrt{\mathbb{E}[\norm{d}_2^2]} =  \sqrt{\inp{\norm{d}_2^2}{\mu^d}}$. The noise process may be constrained to have unit $L_2$ norm by imposing the moment constraint $\inp{\norm{d}_2^2}{\mu^d} = 1$ on $\mu^d$. $L_p$ norms with rational $p > 1$ can be handled with liftings to higher powers \cite{alizadeh2003second}. The $L_1$ norm can be realized by splitting $d(t) = d_+(t) - d_-(t) \in \Delta$ for $d_+, d_- \in \R_+^{N_d}$, with an effective norm $ \norm{d(t)}_1 = \inp{d_+ + d_-}{\mu^d}$.
% the $L_2$-norm of the process $d(t)$ % may be set to a value $e$ by imposing that $\norm{d(t)}_2^2 = \inp{\norm{d}_2^2}{\mu} = e^2$. 
A set of $N_h$ disturbance constraints $\{\int_{t=0}^T h_i(d(t)) dt = e_i\}_{i=1}^{N_h}$ may be imposed by adding constraints to \eqref{eq:peak_meas_un}
\begin{equation}
\inp{h_i(d)}{\textstyle\sum_{k} \mu_{k}} = e_i \quad  \forall i = 1, \ldots, N_h \label{eq:peak_meas_un_int}\\
\end{equation}

The addition of these disturbance constraints forms new dual variables $\lambda \in \R^{N_h}$. The new objective replacing  \eqref{eq:peak_cont_un_obj} is, 
\begin{equation}
    \min_{\gamma \in \R} \quad \gamma + \sum_{i=1}^{N_h} \lambda_i e_i,
\end{equation}
and the flow constraint \eqref{eq:peak_cont_un_flow} becomes, 
\begin{equation}
\Lie_{f_{0k}} v(t, x, w) + \textstyle \sum_{\ell} \zeta_{k \ell} + \textstyle \sum_i \lambda_i h_i(d) \leq 0.
\end{equation}

The same process occurs for a discrete system, where the constraint $\sum_{t=0}^T h(d_t)$ is transformed into the occupation measure constraint $\inp{h}{\mu^d}$. The objective \eqref{eq:peak_cont_un_disc_obj} becomes,
\begin{equation}
    \min \quad \gamma - T \alpha  + \sum_{i=1}^{N_h} \lambda_i e_i,
\end{equation}
and the disturbance constrained discrete flow constraint of \eqref{eq:peak_cont_disc_flow} is,
\begin{equation}
    v(f_k(x), w) -v(x, w)  + \textstyle\sum_i \lambda_i h_i(d)  \leq  \alpha
\end{equation}

% \urg{state inflation, Lipschitz disturbances}
\subsection{Continuity}
Continuity structure may be imposed on the disturbance process $d(t)$ by adding new states to the system (state inflation). As an example, assume that $d(t) \in \Delta = [d_{min}, d_{max}] \in \R, \  \forall t \in [0, T]$ is a 1-dimensional time-varying disturbance process influencing a dynamical system $\dot{x} = f(t, x, d)$. The process $d(t)$ can change arbitrarily quickly in time and has no assumptions of continuity. A derivative (slew rate) constraint $\abs{d'(t)} \leq L$ for some $L \in [0, \infty)$ enforces $C^1$ continuity of the process $d(t)$. The derivative-constrained noise may be realized by adding a new state $y \in \Delta$ such that $x' = f(t, x, y)$ where $y$ is the current value of the disturbance process. The dynamics of $y$ are $y'(t) = d_1(t)$, where $d_1(t)$ is a time varying noise process in the domain $[-L, L]$.

% Two new disturbance processes $d_+(t), \ d_-(t) \in [0, L]$ describing the arbitrarily varying bounded derivatives of the original disturbance. The dynamics of  $y$ are a switched system to ensure that $y \in [d_{min}, d_{max}]$,
% \begin{equation}
% \label{eq:state_inflation}
%     y' = \begin{cases}d_+(t) & y \leq d_{min} \\
%     d_+(t) - d_-(t) & d_{min} \leq y \leq d_{max} \\ 
%     -d_-(t) & y \geq  d_{max}.
%     \end{cases}
% \end{equation}


% \urg{Implement this? Likely to see numerical issues

% I think this is actually a hybrid system, where $y = d_{min}$ and $y = d_{max}$ are guards. Another reason to work on peak estimation for hybrid systems (besides local measures and low-degree approximation). This continuity content should not be used in the paper.
% }

% \urg{Get rid of the $h$ and $\lambda$ terms from the rest of paper, put in here.}

==> sections_arxiv_additional/linear_applications.tex <==
\section{Linear Peak Applications}

\label{sec:linear_app}

This section reviews how peak estimation can be used to bound the maximum absolute value of the impulse response and control effort of MIMO systems.

\subsection{Maximizing Multiple Objectives}

The impulse response and maximum control described later in this section may be realized as linear peak estimation programs \eqref{eq:peak_traj_lin} maximizing $p(x) = \max_i p_i(x)$ for $i = 1, \ldots, N_p$. The objective $p(x)$ can be bounded by solving program \eqref{eq:peak_meas_lin} for each objective $p_i(x)$ yielding upper bounds $p_{id}$. The resultant  bound to $p(x)$ is the maximum upper bound such that $p_{d}^* = \max_{i} p_{id}^*$.

An alternative approach is to maximize $p(x)$ by splitting the peak measure $\mu_p$ as $\sum_{i} \mu_{pi}$. Each split measure satisfies $\mu_{pi} \in \Mp{[0, T] \times X \times W}$. The primal-dual terms of \eqref{eq:peak_meas_lin_obj} and \eqref{eq:peak_cont_lin_p} may be expressed as,
\begin{equation}
    \max \quad \sum_{i=1}^{N_p} \inp{p_i}{\mu_{pi}} \qquad \qquad \qquad v(t, x, w) \geq p_i(x) \quad \forall (t, x, w) \in [0, T] \times X \times W, \ \forall i = 1, \ldots, N_p
\end{equation}

Optimizing over each $p_i$ individually requires solving $N_p$ separate problems. Splitting the peak measure $\mu_p$ into $\sum_i \mu_{pi}$ adds $N_p - 1$ nonnegativity constraints to the original single problem. The max-$i$ and split problems have the same optimum in the infinite dimensional linear program. At a finite degree relaxation the split problem will generally result in a higher bound than the max-$i$, because there is a single $v$ rather than a separate $v$ for each $p_i$. The split problem may be more reasonable to use when there are a large number of measures $(\mu_k, \sigma_{k \ell}, \hat{\sigma}_{k \ell})$ that would otherwise need to be duplicated with max-$i$.



An absolute penalty $\abs{c x}$for some vector $c \in \R^{1 \times N_x}$ may be realized as a max multiple objective peak estimation problem with $p(x) = \max (c x, -cx)$. This expression would not result in an block-diagonalizable invariant semidefinite program, as the function $c(-x) \neq c(x)$. The squared objective $(cx)^2$ is invariant under the transformation $x \rightarrow -x$, and a bound $P^*$ for $\abs{cx}$ may be computed by taking the square root of the upper bound $P^{2*}$ for $(c x)$.
If all objective functions $p_i(x)$ are even (including squared absolute values) then the invariant structure from section \ref{sec:even} may be used to simplify split and max-$i$ LMIs.

\subsection{Impulse Response Analysis}

One application of peak estimation for linear systems is estimating the maximum absolute value of the impulse response across all input/output pairs of a MIMO system \cite{chesi2019computation, chesi2020peak}. 

\subsubsection{Problem Setup}
The system $\dot{x} = Ax + Bu, \ y = C x$ has $N_x$ states, $N_y$ outputs, and $N_u$ inputs. 
The following assumptions are made:
\begin{itemize}
    \item $A_k(t, x, w, d, b)$ is a matrix of size $N_x \times N_x$ for each state $k$,  and dynamics may be decomposed into matrices $\{A_{k \ell}\}$ by \eqref{eq:lin_dynamics_aff}.
    \item $B$ and $C$ are functions strictly of $w$.
\end{itemize}

Define $\{B_j(w)\}_{j=1}^{N_u}$ as the columns of $B$ and $\{C_i(w)\}_{i=1}^{N_y}$ as the rows of $C$ for $i = 1 \ldots N_y$. If the system starting at $x(0) = 0$ receives an impulse at channel $j: \ u = \delta_j$, then the state immediately following this impulse is $x(0^+) = B_j(w)$. The corresponding trajectory is $x_j(t) = x(t \mid x_0 = B_j(w), w, d(t), b(t))$ for a given switching sequence and $d(t), b(t)$. A mixed input $u = \sum c_j \delta_j$ for weights $c_j \in \R^{N_u}, \ \sum_{j=1}^{N_u} c_j = 1$ will result in a trajectory $x(t) = \sum_{j=1}^{N_u} c_j x_j(t \mid x_0 = B_j(w), w, d(t), b(t))$. The set of plausible initial conditions $X_0$ of an impulse response is the convex hull of $\{B_j(w)\}_{j=1}^{N_u}$ for all $w \in W$.


For an output $i$, let $P^{2*}_i$ be the maximum value of the function $(C_i(w) x)^2$ along trajectories starting from $X_0$ (max-$i$). The maximum absolute value of the impulse response $P^*$ may be found,
\begin{equation}
    P^* = \max_i \sqrt{P^{2*}_i}
\end{equation}

% \urg{work on this later}

Program \eqref{eq:peak_meas_lin} with convex and even objective $p(x) = (C_i(w) x)^2$ may be used to upper bound the value $P^{2*}_i$. The initial condition $x^j = B_j(w) \in X, \forall w \in W$ is a function of $w$, and problems \eqref{eq:peak_meas_lin} and \eqref{eq:peak_cont_lin} must be changed accordingly. The invariant initial measure $\mu_0$ of the Liouville \eqref{eq:peak_meas_lin_flow} has the form,
\begin{equation}
\label{eq:even_w_init}
    \frac{1}{2}\left(\sum_{j = 1}^{N_0} \delta_{t = 0} \otimes(B_j(w), w)_\# \mu_{wj} +\delta_{t = 0} \otimes (-B_j(w), w)_\# \mu_{wj}\right)
\end{equation}
% Constraint \eqref{eq:peak_meas_lin_flow} is replaced by,
% \begin{align}
%         & \mu_p = \textstyle\sum_{j = 1}^{N_0} \delta_{t = 0} \otimes (B_j(w), w)_\# \mu_{wj} + \textstyle\sum_{k} \pi^{txw}_\#\Lie_{A_{k0} x}^\dagger \mu_{k} + \pi^{txw}_\#\textstyle\sum_{k\ell} ((A_{k \ell} x) \cdot \nabla_x)^\dagger \sigma_{k \ell}, & \label{eq:peak_meas_lin_flow_w}
% \end{align}
and the $x_j$ in constraint \eqref{eq:peak_cont_lin_init} is substituted,
\begin{equation}
    \quad {\gamma} \geq \frac{1}{2}\left(v(0, B_j(w), w) - v(0, -B_j(w))\right) = v(0, B_j(w), w) \qquad \qquad \forall w \in W, \ j = 1, \ldots, N_u \label{eq:peak_cont_lin_init_w}\\
\end{equation}



\cite{chesi2020peak} details an extensive treatment of an LMI approach towards bounding the impulse response of linear system with polytopic uncertainty. The linear system may switch between $\dot{x} = A_k x + B_k u, \ y = C_k x$ where the $B$ and $C$ matrices are also switching. This setting may be considered as a case of impulse-response estimation with larger $B$ and $C$ matrices formed by concatenating the $B_k$ along columns and $C_k$ along rows. The extended system would have $N_u N_s$ inputs, $N_y N_s$ outputs, and $N_x$ states. This is a slight relaxation as initial inputs cannot be applied to more than one $B_k$ at once. 
Convexity of $(C_{kj} x)^2$ implies that the optimal trajectory will start from at least one pure input $u = B_{kj}$, so the optimum value does not change by combining inputs $B_k$ together.

% The maximum absolute value of the impulse response may be equivalently computed by maximizing 

% \subsubsection{Polytopic Only}

% \cite{chesi2019peak} details an extensive treatment of an LMI approach towards bounding the impulse response of linear system with polytopic uncertainty. A MIMO linear system under polytopic uncertainty may be equivalently expressed as a system with arbitrary switching between $N_s$ subsystems,
% \begin{align}
%     \dot{x} &= A_k x + B_k u\\
%     y &= C_k x.
% \end{align}

% Define $B_{ki}$ and $C_{kj}$ as the $j$th column of $B_k$ and the $j$th row of $C_k$ respectively. At time $t = 0^+$, the set of plausible initial conditions is the convex hull of points $\{B_{ki}\}$. The aim of optimization is to find a tight upper bound on the maximum absolute value of the output $y$. The true value of the peak impulse response is $P^* = \max_{k j} \abs{C_{kj}^T x}$. Because switches are arbitrarily fast, a system may follow dynamics in state $k$, and then instantaneously change to state $k'$ to record a peak output $\abs{C_{k'j} x}$ before returning to state $k$.

% This problem instance may be posed as an instance of \eqref{eq:peak_meas_lin} where only polytopic uncertainty is present. 
% The infinite-time (time-independent) measure program with variables $(c_{ki}, \mu_{pkj}, \mu_k)$ for output $C_{kj}$ is,

% \begin{subequations}
% \label{eq:peak_meas_impulse}
% \begin{align}
%     p_{j}^{2*} = & \  \textrm{max} \quad \inp{(C_{kj} x)^2}{\mu_{p}}&  \\
%     &  \mu_p =  \textstyle\sum_{k=1}^{N_s}\Lie_{A_k x}^\dagger \mu_k + \textstyle\sum_{i=1}^{N_u}c_{ki} \delta_{x = B_{ki}}& \label{eq:peak_meas_impulse_flow}\\
%     & \mu_p, \ \mu_k \in \Mp{X}  & \forall k = 1, \ldots, N_s\\
%     & c_{ki} \in \R_+^{N_u N_s}, \quad \textstyle\sum_{i, k} c_{ki} = 1
% \end{align}
% \end{subequations}

% The Lagrangian of Program \eqref{eq:peak_meas_lin} with dual variables $\psi \in \R^{N_0}_+$ against variables $c$ in \eqref{eq:peak_meas_lin_init} is:
% \begin{align}
%     \label{eq:linear_lagrangian}
%     L &= \inp{(C_{kj} x)^2}{\mu_p} + \inp{v(t,x,w)}{\textstyle\sum_{k, i} c_{ik} \delta_{x = B_{ki}} + \textstyle\sum_{k} \Lie_{A_{k0} x}^\dagger \mu_{k} - \mu_p} \nonumber\\
%   &+ \textstyle \sum_{j=1}^{N_0} c_j \psi_j
%     + \gamma(1 -\inp{1}{\mu_{wj}}) \nonumber .
% \end{align}

% The dual program after absorbing $\phi$ into inequality constraints is,
% \begin{subequations}
% \label{eq:peak_cont_impulse}
% \begin{align}
%     d^{2*}_{j} = & \ \textrm{min}_{\gamma \in \R} \quad \gamma & \\
%     & \gamma \geq v(B_{ki}) & & \forall k, i \\
%     & (A_k x) \cdot \nabla_x v(x) \geq 0 & & \forall x \in X, \ \forall k \label{eq:peak_cont_impulse_f}\\
%     & v(x) + (C_{kj} x)^2 \leq 0 & & \forall x \in X, \forall k \label{eq:peak_cont_impulse_p}\\
%     &v(x) \in C^1(X)
% \end{align}
% \end{subequations}

% The peak measure $\mu_p$ may be broken into $N_y N_s$ separate measures $\mu_{pkj}$ to handle all of the penalties $\abs{C_{k'j} x}$ such that $\mu_p = \sum_{k, j} \mu_{pkj}$. This would require the solution of only one LMI rather than an $N_s N_y$ LMIs (for each $kj$), but would impose $N_s N_y$ nonnegativity constraints on the function $v(x)$ per \label{eq:peak_cont_impulse_p}.

% Problem \eqref{eq:peak_meas_impulse} may be solved over a finite time by adding a constraint $\sum_{k=1}^{N_s} \mu_k \leq T$, just as in the discrete section \ref{sec:discrete}.

% \urg{Considerations of convergence, finite time, certificates, computational efficiency compared to Chesi, etc. The LMIs are simpler and have fewer terms and constraints. }


% Computation of $p^*$ has a runtime which is jointly linear in $N_y$ and $N_u$ and is combinatorial in $N_x$.


\subsubsection{Examples}

\urg{figures and examples go here. Need to fix my code and manually set yalmip to do the invariant measures. I don't know if gloptipoly can automatically handle invariant measures/sign symmetries.}





% For each output $B_j/C_i$ the bound $p^{2*}_{ij}$ is the square of the maximum absolute value of the impulse response. This quantity may be computed by:

\subsection{Maximum Control}
Another problem is finding the maximum state-feedback control effort for a linear system, as treated in \cite{rotondo2020saturation}. Assume that a state feedback controller $u = Kx$ with rows $K_j$ is provided to the linear system $\dot{x} = Ax + Bu$. The closed loop dynamics are $\dot{x} = A^{c\ell} x = (A + B K)x$ with output $y = K x$. Finding the maximum control effort for trajectories starting at some initial set $X_0$ is a peak estimation task with objectives $p_i(x) = \abs{K_i x}$. 


% Just like in impulse response estimation, the computed bound $p^* = \max_j p_j^{2*}$ is accumulated from all rows $K_j$ individually. 
% If $X_0$ is polytopic with $N_0$ vertices, the max-control problem on channel $j$ can be decomposed into $N_0$ separate problems based on the vertices of $X_0$. 

% All linear system programs in this section remain valid for switched systems $\dot{x} = A_k x$ where $X^k = X$. This is due to linearity in dynamics when a switching sequence is fixed \cite{chesi2019ltv}. Problem \eqref{eq:peak_meas_impulse} has $\mu = \sum_k \mu^k$ as in Section \ref{sec:uncertain_switch}, and Constraint \eqref{eq:peak_cont_impulse_f} has $\inp{\nabla_x v(x)}{ A_k x}$ for each $k$. The max-control program has closed-loop matrices $A^{c\ell}_k = A_k + B K$. 


% \subsection{Maximum Control Effort}

% The peak estimation problem can be simplified in the case of linear dynamics  Begin by considering $\dot{x} = f(x) = A x$ where $X_0$ is polytopic with vertices



% Solves the same task as . 

% This is the only comparable paper i've seen so far. Will need to look further.

==> sections_arxiv_additional/linear_system.tex <==
\section{Linear Systems}
\label{sec:linear}
% \urg{I'm not sure if this can be spun off into its own paper. If it stays, add it to the introduction. This should be formatted in a more rigorous fashion, it is currently written like my notes.}

The structure of linear systems may simplify the LMIs necessary to bound extreme values of $p(x)$. The specific linear-in-state dynamics considered in this section are,

\begin{equation}
\label{eq:lin_dynamics}
    \dot{x} = f(x) = A_k(t, w, d, b) x \qquad \qquad \textrm{switching with } X^k = X \ \forall  k = 1, \ldots, N_s.
\end{equation}
It is required that all switching subsystems are valid ($X^k = X$) to ensure linearity of dynamics in all $X$. Dynamics in \eqref{eq:lin_dynamics} may be expanded by box-affine structure into,
\begin{equation}
    \label{eq:lin_dynamics_aff}
    \dot{x} = A_k(t, w, d, b)x = A_{k0}(t, w, d) x + \textstyle\sum_{\ell = 1}^{N_b} b_\ell A_{k \ell}(t, w, d) x .
\end{equation}
The uncertain peak estimation to maximize a function $p(x)$ with dynamics in \eqref{eq:lin_dynamics_aff} over sets $([0, T], X_0, X, W, \Delta)$ may be accomplished by relaxing program \eqref{eq:peak_meas_un} to the finite degree \eqref{eq:peak_lmi_un}. It is assumed that the set $X$ is invariant with respect to trajectories starting from $X_0$ over the time horizon $[0, T]$. 

One common problem setting is when the initial set $X_0$ is a polytope formed by the convex hull of vertices $\{x^j\}_{j=1}^{N_0}$ where $N_0 \leq \infty$. Any $x_0 \in X_0$ be can be expressed as $\sum_{j=1}^{N_0} c_j x^j$ where the weights $c \in \R^{N_0}_+$ satisfy $\sum_{j=1}^{N_0} c = 1$. A trajectory starting at $x_0$ may be decomposed as $x(t \mid x_0, w, d(t)) = \sum_{j=1}^{N_0} c_j x(t \mid x^j, w, d(t))$ by linearity. The ground-truth peak estimation program with convex polytopic $X_0$ may be restated using linearity as,
\begin{align}
\label{eq:peak_traj_lin}
P^* = & \max_{t,\, c ,\,  w ,\,  d(t)}  p(\textstyle \sum_{j=1}^{N_0} c_j x(t \mid x^j, w, d(t))) &\\
& \dot{x}_k(t) = A_{k0}(t, w, d) x + \textstyle\sum_{\ell = 1}^{N_b} b_\ell A_{k \ell}(t, w, d) x & t \in [0, T] \nonumber \\
&d(t) \in \Delta, \ b(t) \in [0, 1]^{N_b} & t \in [0, T] \nonumber \\
& w \in W, \  c \in \R_+^{N_0}, \ \textstyle\sum_{j=1}^{N_0} c_j = 1. \nonumber
\end{align}


Further structure may be exploited by analyzing properties of the objective $p(x)$. Convexity of $p(x)$ implies that
$p(x(1-\lambda) + \lambda(y)) \leq (1-\lambda) p(x) + \lambda p(y), \ \forall x, y \in X, \lambda \in [0, 1]$ by Jensen's inequality. 
This inequality carries over to trajectories, 
\begin{equation}
    \label{eq:linear_convex}
    p(\sum_{j=1}^{N_x} c_j x(t \mid x^j, w, d(t))) \leq \sum_{j=1}^{N_x} c_j p(x(t \mid x^j, w, d(t))) \leq \max_{j} p(x(t \mid x^j, w, d(t))) \qquad \forall t \in [0, T]
\end{equation}
The maximum $P^*$ will therefore be attained at a trajectory starting at one of the corners $x^j$. Problem \eqref{eq:peak_traj_lin} can therefore be split up into $N_0$ problems each starting at point $x^j$ ($c_j = 1, c_{j' \neq j} = 0\}$ and returning bounds $P^*_j$. The final $P^*$ is the maximum $P^*_j$ over all $j$.

A more general structure to the objective is if $p(x)$ is even such that $p(x) = p(-x)$. The linear dynamics in \eqref{eq:lin_dynamics} are equivariant to the transformation $x \rightarrow -x$, as $A(-x) = -(Ax)$. The initial set $X_0$ may be freely chosen to be the convex hull of $\pm x^j$ because 
\begin{equation}
   p(x(t \mid -x^j, w, d(t)) = p(-x(t \mid x^j, w, d(t)) =  p(x(t \mid x^j, w, d(t)).
\end{equation}


% The peak estimation task to maximize a convex $p(x)$ along trajectories starting in $X_0$ in times $[0, T]$ following linear dynamics in \eqref{eq:lin_dynamics_aff} is equivalent by \eqref{eq:linear_convex} to the following program,


% 





% This section analyzes the peak estimation problem of maximizing an objective $p(x)$ over  dynamics $\dot{x} = f(x) = A_k(t, w, d, b) x$ where $A_k$ is the uncertain linear dynamics at switching state $k$. 
% The peak estimation problem can be simplified if $p(x)$ is an even function and $X_0$ is a convex polytope
% formed by the convex hull of vertices $\{x^j\}_{j=1}^{N_0}$ where $N_0 \leq \infty$, and $X$ is known to be an invariant set with respect to $X_0$.

% \subsection{Linear Peak Estimation Problem}
% \urg{convexity not needed, is a bonus. evenness is}
% The following analysis does not exploit affine uncertainty structure, and is general to arbitrary disturbance processes $d(t)$. Convexity of $p(x)$ implies $\forall t \in [0, T]$:


% The maximum value of $p(x)$ along trajectories will therefore be attained at  a vertex $x^j$ for some possibly non-unique $j$. 
% % This result can be specialized to switching and box-type uncertainties by the methods of Section \ref{sec:affine}. Assume that there exists matrices $A_{k \ell}(t, w, d)$ of size $N_x \times N_x$ such that the possibly switched linear dynamics may be expanded into,

\subsection{Linear Measure Program}
Let $\mu_{wj} \in \Mp{W}$ be measures distributed over the uncertain parameters $w \in W$ for each corner point $x^j$ with $j = 1, \ldots, N_0$. The mass $\inp{1}{\mu_wj}$ takes the place of the weight $c_j$
A measure relaxation of Problem \eqref{eq:peak_traj_lin} with variables $(\mu_p, \mu_{wj}, \mu_k, \sigma_{k\ell}, \hat{\sigma}_{k \ell})$ is,


% \urg{I forgot about uncertainty $w$. Need to add that, would require changing everything. The variable is no longer $c_j$ in $c_j (\delta_{t = 0} \otimes\delta_{x = x^j})$, it is now $\mu_{wj}$ in $\delta_{t = 0} \otimes\delta_{x = x^j} \otimes \mu_{wj}$.}

\begin{subequations}
\label{eq:peak_meas_lin}
\begin{align}
p^* = & \ \textrm{max} \quad \inp{p(x)}{\mu_p} & \label{eq:peak_meas_lin_obj} \\
    & \mu_p = \textstyle\sum_{j = 1}^{N_0} \delta_{t = 0} \otimes\delta_{x = x^j} \otimes \mu_{wj} + \textstyle\sum_{k} \pi^{txw}_\#\Lie_{A_{k0} x}^\dagger \mu_{k}  \nonumber&\\
    &\quad \, + \pi^{txw}_\#\textstyle\sum_{k\ell} ((A_{k \ell} x) \cdot \nabla_x)^\dagger \sigma_{k \ell} & \label{eq:peak_meas_lin_flow}\\
    & \textstyle\sum_{j=1}^{N_0} \inp{1}{\mu_{wj}} = 1& \label{eq:peak_meas_lin_prob}\\
    & \sigma_{k \ell} + \hat{\sigma}_{k \ell} = \mu_k &\forall k, \; \ell\label{eq:peak_meas_lin_cont}\\
    & \mu_{k}, \ \sigma_{k \ell}, \ \hat{\sigma}_{k \ell} \in \Mp{[0, T] \times X \times W \times \Delta} &\forall k, \; \ell\\
    & \mu_p \in \Mp{[0, T] \times X \times W} & \\
    & \mu_{wj} \in \Mp{W} & \forall j& \label{eq:peak_meas_lin_init}
\end{align}
\end{subequations}

Problem \eqref{eq:peak_meas_lin} is a specialization of problem \eqref{eq:peak_meas_un}. 
The initial measure is expressed in terms of the vertices $x^j$ as $\mu_0 = \sum_{j = 1}^{N_0} \delta_{t = 0} \otimes\delta_{x = x^j} \otimes \mu_{wj}$. 
The initial measure may be left unchanged as $\mu_0 \in \Mp{X_0 \times W}$ if desired, especially if $X_0$ has a large number of vertices. 
In case there are no uncertain parameters in the system, the variables $\mu_{wj} \in \Mp{W}$ may be replaced by nonnegative scalar weights $c_j \geq 0$. Constraint \eqref{eq:peak_meas_lin_prob} would then read that $\sum_{j=1}^{N_0} c_j = 1$.

% The objective \eqref{eq:peak_meas_lin_obj} involves a single peak measure $\mu_p$, because splitting up $\mu_p$ into the sum of measures $\mu_{pj}$ would be computationally inefficient as $N_0$ grows
\subsection{Linear Function  Program}

The Lagrangian of Program \eqref{eq:peak_meas_lin} is:
\begin{align}
    \label{eq:linear_lagrangian}
    L &= \inp{p(x)}{\mu_p} + \inp{v(t,x,w)}{\textstyle\sum_{j = 1}^{N_0} (\delta_{t = 0} \otimes\delta_{x = x^j} \otimes \mu_{wj}) + \textstyle\sum_{k} \Lie_{A_{k0} x}^\dagger \mu_{k}} \nonumber\\
    &+ \inp{v(t,x,w)}{\textstyle\sum_{k\ell}(A_{k \ell} \cdot \nabla_x)^\dagger \sigma_{k \ell} - \mu_p} + \textstyle \sum_{j=1}^{N_0} c_j \psi_j \\
    &+ \gamma(1 -\inp{1}{\mu_{wj}}) + \textstyle\sum_{k \ell} \inp{\zeta_{k \ell}(t, x, w, d)}{\mu_k - \sigma_{k \ell} - \hat{\sigma}_{k \ell} } \nonumber .
\end{align}
% (1 - \inp{1}{\mu_0})

The resultant infinite-dimensional linear function program formed by minimizing the Lagrangian in \eqref{eq:linear_lagrangian} with variables $(v, \gamma, \zeta)$ is,

\begin{subequations}
\label{eq:peak_cont_lin}
\begin{align}
    d^* = & \ \min_{\gamma \in \R} \quad \gamma \label{eq:peak_cont_lin_obj}\\
    & \forall w \in W: \quad \forall j\nonumber \\
    & \quad {\gamma} \geq {v(0, x^j, w)} &   \label{eq:peak_cont_lin_init}\\
    & \forall (t, x, w, d) \in [0, T] \times X \times W \times \Delta: \quad \forall k, \; \ell \nonumber \\
    & \quad \partial_t v(t, x, w) + (A_{k0} x) \cdot \nabla_x v(t, x, w) + \textstyle \sum_{\ell} \zeta_{k \ell}\leq 0 \label{eq:peak_cont_lin_flow}\\
    & \quad (A_{k\ell} x) \cdot \nabla_x v(t, x, w) \leq \zeta_{k \ell} \\
    & \forall (t, x, w) \in [0, T] \times X \times W: \nonumber \\
    & \quad v(t, x) \geq p(x) \label{eq:peak_cont_lin_p}  \\
    &v \in C^1([0, T]\times X \times W) \label{eq:peak_cont_lin_v} \\
    & \zeta_{k \ell} \in C_+([0, T]\times X \times W \times \Delta) \qquad \forall k, \; \ell.
\end{align}
\end{subequations}

% The variable $\psi$ is absorbed into the inequality constraint of \eqref{eq:peak_cont_lin_init}.
When there are no uncertain parameters $w$, constraint \eqref{eq:peak_cont_lin_init} is replaced by,
\begin{equation}
    \gamma \geq v(0, x^j) \qquad  \forall j = 1, \ldots, N_0
\end{equation}


\subsection{Even objective}
\label{sec:even}
Problem \eqref{eq:peak_meas_lin} may be modified to produce an invariant linear program if $p(x)$ is even. The initial measure $\mu_0$ may be replaced by, 
\begin{equation}
\label{eq:even_init}
\mu_0 = \sum_{j = 1}^{N_0} \delta_{t = 0} \otimes \frac{1}{2}(\delta_{x = x^j} + \delta_{x = -x^j}) \otimes \mu_{wj}.
\end{equation}
The initial measure remains a probability measure describing points that start at $x = \pm x^j$. The peak measure $\mu_p$ is likewise invariant, because if a point $x^*$ satisfies $p(x^*) = P^*$ then the negative $-x^*$ also reaches $p(-x^*)=P^*$. The (disturbance) occupation measures all inherit this invariant structure given that the initial measure $\mu_0$ is invariant.

Moment matrices of invariant measures may be block-diagonalized \cite{cimprivc2009sums, riener2013exploiting}. The sizes and multiplicity of the blocks are related to the symmetry group's irreducible representations. If a measure $\mu$ is invariant on the action $x \rightarrow -x$, then the moment $\E_\mu[x^\alpha t^\beta w^\gamma d^\delta]$ vanishes to zero whenever $\abs{\alpha}$ is odd. As an example, the $x_1$ moment of $\delta_{x^j} + \delta_{x=-x^j}$ is $x^j_1 + (-x^j_1) = 0$. Moment matrices $\M[y]$ of this type of invariant measure can be block-diagonalized into $\M^{odd}[y]$ and $\M^{even}[y]$. The rows (and columns) of $\M^{odd}[y]$ are indexed by multi-indices where $\abs{\alpha}$ is odd, while $\M^{even}[y]$ has even $\abs{\alpha}$. 

The full moment matrix $\M_d[y]$ at degree $d$ has size $\binom{n+d}{d}$. The sizes of the two blocks are,
\begin{equation}
    \M^{odd}_d[y]: \ \sum_{d' \textrm{ even}}^{d} \binom{n+d'-1}{d'} \qquad \qquad \M^{even}_d[y]: \ \sum_{d' \textrm{ even}}^{d} \binom{n+d'-1}{d'},
\end{equation}
which together add to $\binom{n+d}{d}$. All measures $(\mu_0, \mu_p, \mu_k, \sigma_{k \ell}, \hat{\sigma}_{k \ell}$ may have their moment matrices block-diagonalized in this fashion, reducing the size of the semidefinite constraint blocks in the LMI.
% All other measures will inherit this even symmetric structure with $x \rightarrow -x$ due to equivariance of dynamics.

The dual problem \eqref{eq:peak_cont_lin} may implement this symmetry by requiring that $v(t, x, w) = v(t, -x, w)$. In the SOS relaxation, $v$ would then be a member of the invariant ring of polynomials with respect to this group action. Such a $v$ has a decomposition into $v^{odd}(t, x, w) + v^{even}(t, x, w)$ as described previously. Constraint \eqref{eq:peak_cont_lin_init} is effectively unaffected, as it is replaced by the equivalent, 
\begin{equation}
    \forall w \in W, \ \forall j = 1, \ldots, N_0: \qquad \gamma \geq \frac{1}{2}(v(0, x^j, w) + v(0, -x^j, w)) = v(0, x^j, w)
\end{equation}
to match the initial measure \eqref{eq:even_init}.


The set of sum-of-squares invariant polynomials is $\sigma^{odd}(t, x, w) + \sigma^{even}(t, x, w)$ where $\sigma^{odd}, \  \sigma^{even}$ are each SOS \cite{gatermann2004symmetry}. Program \eqref{eq:peak_cont_lin} may accomodate the invariant structure by using the invariant decomposition when enforcing the SOS constraints \eqref{eq:peak_cont_lin_flow} - \eqref{eq:peak_cont_lin_p}. The semidefinite Gram matrices describing SOS polynomials $\sigma_d^{odd}, \  \sigma_d^{even}$ are dual to the moment matrices $\M^{odd}_d[y], \ \M^{even}_d[y]$.

==> sections_arxiv_additional/lmi_continuous.tex <==
\subsection{Uncertain LMI}

\label{sec:lmi_cont}
The compact semialgebraic sets in the uncertain peak estimation setting are
\begin{align}
    \label{eq:peak_sets}
    X &= \{x \mid g_i(x)\geq 0 & &\mid \ i = 1, \ldots, N_c\} \\
    X_0 &= \{x \mid  g_{0i}(x)\geq 0 & &\mid \ i = 1, \ldots, N_c^0\}\\
    W &= \{w \mid g_{wi}(w)\geq 0 & &\mid \ i = 1, \ldots, N_c^w\}\\
    \Delta &= \{d \mid g_{di}(d)\geq 0 & &\mid \ i = 1, \ldots, N_c^d\}.
\end{align}

The degree of $g_i(x)$ is $d_i$, and other degrees $d_{0i}, \ d_{wi}, \ d_{di}$ are defined on corresponding polynomials. Monomials forming moments may be indexed as  $x^\alpha t^\beta w^\gamma d^\delta$ for multi-indices $\alpha \in \N^{N_x}, \ \beta \in \N, \ \gamma \in \N^{N_w}, \ \delta \in \N^{N_d}$. Define $y^0 = \{y^0_{\alpha \gamma} \}, \ y^p = \{y^p_{\alpha \beta \gamma}\}$ as the moment sequences for measures $\mu_0$ and $\mu_p$, just as in Section \ref{sec:peak_lmi}. The moment sequence for the occupation measure $\mu^k$ is $y^k = \{y^k_{\alpha \beta \gamma \delta}\}$ for each switching subsystem $k$. The box-affine disturbance occupation measures $\sigma_{k\ell}, \hat{\sigma}_{k\ell}$ likewise have moment sequences $s^{k\ell} = \{s^{k \ell}_{\alpha \beta \gamma \delta}\}, \ \hat{s}^{k \ell} = \{\hat{s}^{k\ell}_{\alpha \beta \gamma \delta}\}$. The Liouville equation \eqref{eq:peak_meas_un_flow} with test function $v(t, x, w) = x^\alpha t^\beta w^\gamma$ has the form,
\begin{equation}
\label{eq:liou_lmi_unc}
    \inp{x^\alpha t^\beta w^\gamma}{ {\delta_0 \otimes} \mu_0} + \textstyle \sum_k\inp{\Lie_{f_{0k}}( x^\alpha t^\beta w^\gamma)}{\mu_k} + \textstyle\sum_{k \ell}\inp{f_{k\ell} \cdot \nabla_x(x^\alpha t^\beta w^\gamma)}{\sigma_{k\ell}} - \inp{x^\alpha t^\beta w^\gamma}{\mu_p} = 0.
\end{equation}
Define the operator $\textrm{Liou}_{\alpha \beta\gamma }(y^0, y^p, y^k, s^{k \ell})$ as the linear relation between the moment sequences induced by \eqref{eq:liou_lmi_unc}, just as in problem \eqref{eq:peak_lmi}.
The degree-$d$ LMI relaxation of the uncertain peak estimation problem in  \eqref{eq:peak_meas_un} resulting in an upper bound $p^*_d \geq P^*$ is, 
\begin{subequations}
\label{eq:peak_lmi_un}
\begin{align}
    p^*_d = & \textrm{max} \quad \textstyle\sum_{\alpha} p_\alpha y_{\alpha 0 0}^p \label{eq:peak_lmi_un_obj} \\
    & \textrm{Liou}_{\alpha \beta \gamma}(y^0, y^p, y^k, s^{k \ell}) = 0 \quad \textrm{by \eqref{eq:liou_lmi_unc}} & &  \forall \abs{\alpha} + \abs{\beta} + \abs{\gamma} \leq 2d \label{eq:peak_lmi_un_flow}\\
    & y^0_0 = 1 \\
    & \forall k \ell: s^{k \ell}_{\alpha \beta \gamma \delta} + \hat{s}^{k \ell}_{\alpha \beta \gamma \delta}  = y^k_{\alpha \beta \gamma \delta}  & &  \forall \abs{\alpha} + \abs{\beta} + \abs{\gamma} + \abs{\delta} \leq 2d \label{eq:peak_lmi_un_abscont}\\
    & \M_d(y^0), \M_d(y^p), \forall k: \M_d(y^k) \succeq 0 \label{eq:peak_lmi_un_psd} \\
    & \forall k \ell: \M_d(s^{k \ell}), \M_d(s^{k \ell}) \succeq 0 \label{eq:peak_lmi_un_psd_box} \\
    &\M_{d - d_{0i}}(g_{0i} y^0) \succeq 0  \label{eq:peak_lmi_un_init}  & &\forall i = 1, \ldots, N_c^0\\ 
    &\M_{d - d_{wi}}(g_{wi} y^0) \succeq 0  \label{eq:peak_lmi_un_init_w}  & &\forall i = 1, \ldots, N_c^w\\ 
    &\M_{d - d_i}(g_{i} y^p), \ \forall k: \M_{d - d_i}(g_{i} y^k) \succeq 0 & & \forall i = 1, \ldots, N_c \\ 
    &\forall k \ell: \ \M_{d - d_i}(g_{i} s^{k \ell}), \ \M_{d - d_i}(g_{i} \hat{s}^{k \ell}) \succeq 0  & & \forall i = 1, \ldots, N_c  \label{eq:peak_lmi_un_state} \\
    &\M_{d - d_{wi}}(g_{wi} y^p), \ \forall k: \M_{d - d_{wi}}(g_{wi} y^k) \succeq 0 & & \forall i = 1, \ldots, N_c^w \\ 
    &\forall k \ell: \ \M_{d - d_{wi}}(g_{wi} s^{k \ell}), \ \M_{d - d_{wi}}(g_{wi} \hat{s}^{k \ell}) \succeq 0  & & \forall i = 1, \ldots, N_c^w  \label{eq:peak_lmi_un_w} \\
    &\M_{d-2}(t(T-t)y^p), \forall k: \M_{d-2}(t(T-t)y^k) \succeq  0 \label{eq:peak_lmi_un_supp2} \\
    & \forall k \ell: \ \M_{d-2}(t(T-t)s^{k \ell}), \  \M_{d-2}(t(T-t)\hat{s}^{k \ell}) \succeq 0 & &   \\
    &\forall k: \M_{d - d_{di}}(g_{di} y^k) \succeq 0 & & \forall i = 1, \ldots, N_c^d \\ 
    &\forall k \ell: \ \M_{d - d_{di}}(g_{di} s^{k \ell}), \ \M_{d - d_{di}}(g_{di} \hat{s}^{k \ell}) \succeq 0  & & \forall i = 1, \ldots, N_c^d \label{eq:peak_lmi_un_d}
\end{align}
\end{subequations}

Many of the constraints and definitions are similar to the standard peak estimation problem in \eqref{eq:peak_lmi}. Constraint \eqref{eq:peak_lmi_un_abscont} enforces the absolute continuity condition $\sigma^{k \ell} + \hat{\sigma}^{k \ell} = \mu^k$ in \eqref{eq:peak_meas_un_abscont}. Constraints \eqref{eq:peak_lmi_un_psd}- \eqref{eq:peak_lmi_un_d} are moment and localizing matrix PSD constraints ensuring that there exist representing measures to the moment sequences $(y^0, y^p, y^k, s^{k \ell}, \hat{s}^{k \ell})$ supported on the appropriate spaces.





==> sections_arxiv_additional/prelim_lmi_peak.tex <==
\subsection{Peak Estimation LMI}

\label{sec:peak_lmi}
The peak estimation problem \eqref{eq:peak_meas} may be approximated through a moment LMI. 


Let $(y^0, y^p)$ represent moment sequences up to order $2d$ of the measures $\mu$, and $y$ be moment sequences up to order $2(d + \textrm{deg}(f) -1)$ of the occupation measure $\mu$.
The Liouville equation in \eqref{eq:peak_meas_flow} induces a linear relation between the moment sequences $(y^0, y, y^p)$ for the test function $x^\alpha t^\beta$,
\begin{equation}
\label{eq:liou_mom_lmi}
    \inp{x^\alpha t^\beta}{ {\delta_0 \otimes} \mu_0} + \inp{\Lie_f( x^\alpha t^\beta)}{\mu} - \inp{x^\alpha t^\beta}{\mu_p} = 0.
\end{equation}
The expression $\textrm{Liou}_{\alpha \beta}(y^0, y, y^p)$ is defined as this expression at the test function $x^\alpha t^\beta$.
The degree-$d$ moment-LMI relaxation of program  \eqref{eq:peak_meas} is, 
\begin{subequations}
\label{eq:peak_lmi}
\begin{align}
    p^*_d = & \textrm{max} \quad \textstyle\sum_{\alpha} p_\alpha y_{\alpha 0}^p. \label{eq:peak_lmi_obj} \\
    & \textrm{Liou}_{\alpha \beta}(y^0, y, y^p) = 0 \quad \textrm{by \eqref{eq:liou_mom_lmi}} \forall (\alpha, \beta) \in \N^{n+1}_{\leq 2d} \label{eq:peak_lmi_flow}\\
    & y^0_0 = 1 \\
    & \M_d(y^0), \M_d(y), \M_d(y^p) \succeq 0 \label{eq:peak_lmi_psd} \\
    &\M_{d - d_{0i}}(g_{0i} y^0) \succeq 0  \label{eq:peak_lmi_init} & &\forall i = 1, \ldots, N_c^0\\ 
    &\M_{d - d_i}(g_{i} y) \succeq 0 & & \forall i = 1, \ldots, N_c \label{eq:peak_lmi_peai} \\ 
    &\M_{d - d_i}(g_{i} y^p) \succeq 0 & &\forall i = 1, \ldots, N_c \\ 
    &\M_{d-2}(t(T-t)y),   \ \M_{d-2}(t(T-t)y^p) {\; \succeq \;} 0. \label{eq:peak_lmi_supp2}
\end{align}
\end{subequations}

The formulation in \eqref{eq:peak_lmi} assumes that $X = \{g_i(x)\geq 0 \mid \ i = 1, \ldots, N_c\}$ and $X_0 = \{g_{0i}(x)\geq 0 \mid \ i = 1, \ldots, N_c^0\}$ are both compact (Archimedean) basic semialgebraic sets. Constraints \eqref{eq:peak_lmi_psd}-\eqref{eq:peak_lmi_supp2} enforce that $(y^0, y, y^p)$ are moments corresponding to representing measures $\mu_0 \in \Mp{X_0}$ and $\mu, \mu_p \in \Mp{[0, T] \times X}$. These representing measures may not satisfy the infinite-dimensional Liouville equation in constraint \eqref{eq:peak_meas_flow}, only a finite number of induced Liouville constraints are included in \eqref{eq:peak_lmi_flow}. 

The upper bounds $p_d^*$ will tend towards $P^*$ as $d\rightarrow \infty$ given that $X_0$ and $[0, T] \times X$ are each compact. By theorem C.20 of \cite{lasserre2009moments}, the degree-$d$ LMI problem \eqref{eq:peak_lmi} is strongly dual to the degree-$d$ SOS relaxation of \eqref{eq:peak_cont}. This duality justifies the name Moment-SOS hierarchy, where the `hierarchy' is posed over increasing degree $d$.

% \subsection{Previous Content}

% % The conditions that $y$ are the moments of a nonnegative measure supported over a semialgebraic set $\K$ is dual to the Psatz requirements 


% The infinite moment matrix $\M(y)$ and localizing matrices $\M(g_{k} y)$ for each inequality constraint are indexed by multi-indices $(\alpha, \beta)$, and have the forms,  
% \begin{equation}
%     \M(y)_{\alpha \beta} = y_{\alpha + \beta}, \quad \M(g_{k} y)_{\alpha \beta}  =  \textstyle\sum_{\gamma} g_{k \gamma} y_{\alpha + \beta + \gamma}.
% \end{equation}

% The problem of recovering a probability distribution from a restricted set of moments


% \urg{previous content}
% Infinite-dimensional LPs may be defined over nonnegative measures $\mu$, such as 
% \begin{equation}
% \label{eq:meas_program} p^* =  \max_{\mu \in \Mp{X}} \inp{c}{\mu}, \qquad  \mathcal{A}(\mu) = b.
% \end{equation}
% In program \eqref{eq:meas_program}, $c \in \R[x] \subset C(X)$ is a cost, and $\mathcal{A}, b$ define a set of affine constraints in the moments of $\mu$. 
% % Nonconvex polynomial optimization problems may be reformulated into the form of the convex infinite-dimensional LP in  \eqref{eq:meas_program} \cite{lasserre2009moments}. 
% The $\alpha$-moment of a measure $\mu$ is the scalar quantity $y_\alpha = \inp{x^\alpha}{\mu}$.
% A measure $\mu$ from \eqref{eq:meas_program} may be parameterized by an infinite sequence of moments $y = \{y_\alpha \mid \ \forall \alpha \in \N^n\} $ such that $\inp{p}{\mu} = \sum_{\alpha} p_\alpha y_\alpha$ for all  $p \in \R[x]$.  
% Problem \eqref{eq:meas_program} may be expressed as a linear program in the infinite number of moments $y_\alpha$, which
% must be truncated into a problem with a finite number of variables and constraints for tractable optimization. The moment-sum-of-squares (SOS) hierarchy uses  the moment sequence $y_\alpha$ with degree $\abs{\alpha} \leq d$ for some bound $d$ as variables. Refer to \cite{lasserre2009moments} for all material in this subsection. 

% Let $X = \{x \mid g_k(x) \geq 0\}$ be a basic semialgebraic set with $N_c$ constraints where each $g_k(x)$ has degree $d_k$, and $\alpha, \beta, \gamma \in \N^m$ be a set of multi-indices. 


% % define $\M_d(y)$ as the Moment Matrix of degree $d$ and $\M_{d - d_k}(g_{k} y)$ as the localizing matrices for each inequality constraint.   Precise definitions of $\M(y)$ and $\M(g_X y)$ are in \cite{lasserre2009moments}.
% % \new{(Didier: Should we define formally the moment and localizing matrices, or just refer to the literature ?)}
% The degree-$d$ relaxation of problem \eqref{eq:meas_program} is:
% \begin{subequations}
% \begin{align}
% \label{eq:mom_program}
%     p^*_d &=  \ \max_{y} \textstyle\sum_\alpha c_\alpha y_\alpha, \qquad  A(y) = b_y \\
%     & \M_d(y) \succeq 0, \; \M_{d - d_k}(g_{k} y) \succeq 0  \; \forall i = 1, \ldots, N_c.
% \end{align}
% \end{subequations}
% % \mid_{k=1}^{N_c}

% The truncated moment matrix $\M_d(y)$ and localizing matrices $\M_{d-d_k}(g_k y)$ contain moments of up to order $2d$. The expression $A(y)=b_y$ in problem \eqref{eq:mom_program} imposes the affine condition $\mathcal{A}(\mu) = b$ on entries of the moment sequence $y$.
% The optima of relaxations $p^*_{d} \geq p^*_{d+1} \geq p^*_{d+2} \ldots$ are a sequence of upper bounds to the true optimum $p^*$. 
% % For a polynomial optimization problem, the sequence of upper bounds will converge to $p^*$ at a finite degree $d$
% This sequence will converge as $d \rightarrow \infty$ if $X$ is compact, or more specifically an Archimedean condition holds \cite{lasserre2009moments}. The size of $\M_d(y)$ (size of the PSD matrix variable of an LMI absent other structure) with $n$ variables at degree $d$ is $\binom{n+d}{d}$.
% % The time complexity of LMI solvers are generally polynomial in the size of the PSD matrix variable, which results in combinatorially scaling runtime as $d$ increases.
% % As the performance of LMI solvers is generally polynomial in the size of the PSD matrix variable, the moment-SOS hierarchy [TODO]... 
% % increases as $O(n^d)$, and the complexity of solving \eqref{eq:mom_program} scales combinatorially as $O(n^{6d})$ }.
% % This is verified by a `flat extension' of moment matrices, which is a condition that ensures  the rank $\M_{\delta}(y)$ does not increase as the degree $\delta \leq d$ increases \cite{lasserre2009moments}. A moment sequence

% A measure is `rank-$r$ atomic' if it is supported on a set of $r$ discrete points called `atoms'. A moment matrix $\M_d(y)$ possesses a representing measure $\mu$ if the moments of $\mu$ up to order $2d$ agree with the entries of $\M_d(y)$. 
% A necessary but not sufficient condition for a rank-$r$ atomic measure $\mu$ to exist is that $\M_d(y)$ has rank $r$. The sufficient condition requires the existence of a flat extension, in which the rank of truncated moment matrices is preserved as $d$ increases \cite{laurent2009generalized}.
% % $y$ has a representing measure $\mu$ supported at $r$ points in $X$ if 
% % \old{each $\M_{d - d_k}(g_k) \succeq 0$,}
% % $\M_{d}(y)$ has rank $r$ and the flat extension holds. 
% % Each of the $r$ support points are called `atoms', and $\mu$ is therefore an rank-$r$ atomic measure. 
% The $r$ atoms may be recovered by a Cholesky decomposition of $\M_d(y)$, or by reading entries of $y_\alpha$ if $r=1$ \cite{henrion2005detecting}.

% % When $\mu$ is rank-1 atomic, the location of the only atom may} 
% % and coordinates of $\mu$'s support can 
% % be read from the moment sequence $y_{\alpha}$.
% % for $\abs{\alpha} \leq 1$ if $\M_d(y)$ is rank-1.


==> sections_arxiv_additional/summary_extended.tex <==
This paper has the following structure: Section \ref{sec:preliminaries} reviews preliminaries such as occupation measures and peak estimation. Section \ref{sec:uncertainty} presents uncertainty models, and a unified uncertain peak estimation model is presented in Section \ref{sec:unified}. Section \ref{sec:discrete} extends uncertain peak estimation to discrete systems. 
The specific case of uncertain peak estimation applied to linear systems analysis are detailed in sections \ref{sec:linear} and \ref{sec:linear_app}
Safety analysis is treated using uncertain peak estimation in section \ref{sec:safety}. 
Other extensions of these techniques are mentioned in \ref{sec:extensions}. 
The paper is concluded in section \ref{sec:conclusion}.
